Distributionally Robust Model-Based Offline Reinforcement Learning with Near-Optimal Sample Complexity

This paper concerns the central issues of model robustness and sample efficiency in offline reinforcement learning (RL), which aims to learn to perform decision making from history data without active exploration. Due to uncertainties and variabilities of the environment, it is critical to learn a robust policy -- with as few samples as possible -- that performs well even when the deployed environment deviates from the nominal one used to collect the history dataset. We consider a distributionally robust formulation of offline RL, focusing on tabular robust Markov decision processes with an uncertainty set specified by the Kullback-Leibler divergence in both finite-horizon and infinite-horizon settings. To combat with sample scarcity, a model-based algorithm that combines distributionally robust value iteration with the principle of pessimism in the face of uncertainty is proposed, by penalizing the robust value estimates with a carefully designed data-driven penalty term. Under a mild and tailored assumption of the history dataset that measures distribution shift without requiring full coverage of the state-action space, we establish the finite-sample complexity of the proposed algorithms. We further develop an information-theoretic lower bound, which suggests that learning RMDPs is at least as hard as the standard MDPs when the uncertainty level is sufficient small, and corroborates the tightness of our upper bound up to polynomial factors of the (effective) horizon length for a range of uncertainty levels. To the best our knowledge, this provides the first provably near-optimal robust offline RL algorithm that learns under model uncertainty and partial coverage.

==> discussion.tex <==

\section{Discussions}
\label{sec:discussions}
Focusing on model-free paradigms, this paper has developed near-optimal sample complexities for some variants of pessimistic Q-learning algorithms --- armed with lower confidence bounds and variance reduction --- for offline RL. These sample complexity results, taken together with the analysis framework developed herein, open up a few exciting directions for future research.
 For example, the pessimistic Q-learning algorithms can be deployed in conjunction with their optimistic counterparts (e.g., \citet{jin2018q,li2021breaking,zhang2020almost}), when additional online data can be acquired to fine-tune the policy \citep{xie2021policy}. In addition, the $\varepsilon$-range for \LCBQR to attain sample optimality remains somewhat limited (i.e., $\varepsilon \in (0,1/H])$). Our ongoing work \citet{li2022settling} suggests that a new variant of pessimistic model-based algorithm is sample-optimal for a broader range of $\varepsilon$, which in turn motivates further investigation into whether model-free algorithms can accommodate a broader $\varepsilon$-range too without compromising sample efficiency.   
Moving beyond the tabular setting, it would be of great importance to extend the algorithmic and theoretical framework to accommodate low-complexity function approximation \citep{nguyen2021sample}.  


==> lower-bound-analysis-exp.tex <==
%!TEX root = ./DRO-offline.tex
\section{Proof of Theorem~\ref{thm:dro-lower-finite}} 
\label{proof:thm:dro-lower-finite}
 
The proof of Theorem~\ref{thm:dro-lower-finite} is inspired by the construction of the MDP in \citep{li2022settling}.
We shall first construct some hard instances and then characterize the sample complexity analyses over these instances.

\subsection{Construction of hard problem instances}
\paragraph{Construction of a collection of hard MDPs.} Let us introduce two MDPs
\begin{align}
   \left\{ 
    \big(\mathcal{S}, \mathcal{A}, P^{\phi} = \{P^{\phi}_h\}_{h=1}^H, \{r_h\}_{h=1}^H, H \big) 
    \mid \phi = \{0,1\}
    \right\},
\end{align}
%
where the state space is $\cS = \{0, 1, \ldots, S-1\}$, and the action space is $\mathcal{A} = \{0, 1\}$. 
% Observe that each $\phi\in\Phi$ uniquely determine a MDP $\mathcal{M}^\phi \in \mathsf{MDP}(\Phi)$.
Then we shall introduce the transition kernel $P^\phi$ of the constructed MDP $\cM_\phi$, which is similar to a contexual multi-arm bandits. The transition kernel is defined as
\begin{align}
P^{\phi}_1(s^{\prime} \mymid s, a) = \left\{ \begin{array}{lll}
         p\mathds{1}(s^{\prime} = 0) + (1-p)\mathds{1}(s^{\prime} = 1)  & \text{if} & (s, a) = (0, \phi_h) \\
         q\mathds{1}(s^{\prime} = 0) + (1-q)\mathds{1}(s^{\prime} = 1) & \text{if} & (s, a) = (0, 1-\phi_h) \\
         \mathds{1}(s^{\prime} = 1) & \text{if}   & (s, a) = (1, 0) \\ 
         q\mathds{1}(s^{\prime} = 1) + (1-q) \mathds{1}(s^{\prime} = 0) & \text{if}   & (s, a) = (1, 1) \\ 
         q\mathds{1}(s^{\prime} = s) + (1-q)\mathds{1}(s^{\prime} = 1) & \text{if}   & s > 1 \
                \end{array}\right.
        \label{eq:Ph-construction-lower-finite}
\end{align}
and 
\begin{align}
P^{\phi}_h(s^{\prime} \mymid s, a) = \mathds{1}(s^{\prime} = s),\qquad \forall (h,s,a) \in [H]\setminus \{1\} \times \cS \times \cA.
        \label{eq:Ph-construction-lower-finite-h}
\end{align}





% With the above distribution in mind, we specify the transition kernel $P^{\phi} = \{P^{\phi}_h\}_{h=1}^H$ of the MDP $\mathcal{M}^\phi$ as follows:
% %
% \begin{align}
% P^{\phi}_h(s^{\prime} \mymid s, a) = \left\{ \begin{array}{lll}
%          p\mathds{1}(s^{\prime} = 0) + (1-p)\mu(s^{\prime}) & \text{if} & (s, a) = (0, \phi_h) \\
%          q\mathds{1}(s^{\prime} = 0) + (1-q)\mu(s^{\prime}) & \text{if} & (s, a) = (0, 1-\phi_h) \\
%          \mathds{1}(s^{\prime} = 1) & \text{if}   & (s, a) = (1, 0) \\ 
%          \big(1 - e^{-c_1 H}\big)\mathds{1}(s^{\prime} = 1) + e^{-c_1 H} \mu(s^{\prime}) & \text{if}   & (s, a) = (1, 1) \\ 
%          \big(1 - \frac{1}{H}\big)\mathds{1}(s^{\prime} = s) + \frac{1}{H}\mu(s^{\prime}) & \text{if}   & s > 1 \
%                 \end{array}\right.
%         \label{eq:Ph-construction-lower-finite}
% \end{align}
% %
% for any $(s,a,s',h)\in \cS\times \cA\times \cS\times [H]$. 

Here, $p$ and $q$ are set to be 
%
\begin{equation}
    p = 1 - \frac{c_1}{H} + \Delta
    \qquad \text{and} \qquad
    q = 1 - \frac{c_1}{H}  \label{eq:finite-p-q-def}
\end{equation}
% for some sufficiently large constant $c_1 > 0$.
for some sufficiently large constant $c_1 > 0$ and $\Delta$ (the value of $\Delta$ will be specified later.) obeying 
%
\begin{equation}
    \frac{c_1}{H} \leq \frac{1}{2} \qquad \text{and} \qquad \Delta \leq \frac{c_1}{2H}.
\end{equation}
The above fact immediately indicates the facts
\begin{align}\label{eq:lower-p-q-assumption}
    1> p>q \geq \frac{1}{2}.
\end{align}
Note that based on the current state, the MDP will only transfer to a different state in the time step $h=1$ and shall always stay in the same state in all other time steps $h\in [H] \setminus \{1\}$. Additionally, the agent will always stay in the state subset $\{0,1\}$ if the initial distribution supported only on $\{0,1\}$, in view of \eqref{eq:Ph-construction-lower-finite}.
With abuse of notation, we denote the transition kernel vector as
\begin{align}
    P_{h,s,a}^{\phi} \defn P^{\phi}_h(\cdot \mymid s,a) \in [0,1]^{1\times S}.
\end{align}
%
% It is readily seen from the above assumption that
% %
% \begin{align}
%     p> q \geq \frac{1}{2} .
%     \label{eq:p-q-order-LB-finite}
% \end{align}
To continue, for any $(h,s,a)\in  [H]\times\cS\times \cA$, the reward function of the MDPs are defined as
\begin{align}
r_h(s, a) = \left\{ \begin{array}{lll}
         1 & \text{if } s = 0 \\
         0 & \text{otherwise}  \ 
                \end{array}\right. 
        \label{eq:rh-construction-lower-bound-finite}
\end{align}
%



% Finally, let's specify the set $\Phi$. By virtue of the Gilbert-Varshamov lemma \citep{gilbert1952comparison}, we can construct a set $\Phi \subseteq  \{0, 1\}^{H}$ such that 
% %
% \begin{equation}
%     |\Phi| \ge e^{H/8}
%     \qquad \text{and} \qquad 
%     \|\phi - \widetilde{\phi}\|_1 \ge \frac{H}{8}
%     \quad 
%     \text{for any }\phi,\widetilde{\phi}\in \Phi, \phi \ne \widetilde{\phi}. 
%     \label{eq:property-Theta} 
% \end{equation}

\paragraph{Construction of the history batch dataset.}


In some nominal environment $\cM_\phi$, a batch dataset is obtained consisting of $K$ {\em independent} sample trajectories each of length $H$. Before defining the dataset, letting $\mathds{1}(\cdot)$ be the indicator function, it is convenient to introduce the following state distribution supported on the state subset $\{0,1\}$:
%
\begin{align}\label{finite-mu-assumption}
       \mu(s) = \frac{1}{CS}\mathds{1}(s = 0) + \Big(1 - \frac{1}{CS}\Big)\mathds{1}(s = 1),
\end{align}
%
where $C>0$ is some constant that will determine the concentrability coefficient $\Cstar$ (as we shall detail momentarily) and obeys
\begin{align}\label{eq:lower-C-assumption}
    \frac{1}{CS} \leq \frac{1}{4}.
\end{align}
Suppose the dataset is generated according to \eqref{eq:finite-batch-size-def}, based on the following chosen initial state distribution $\rhob$ and the behavior policy 
$\pib = \{\pib_h\}_{h=1}^H$: 
%
\begin{align}\label{eq:lower-dataset-assumption}
    \rhob (s) = \mu(s)\quad \text{and } \quad\pi_h^{\mathsf{b}}(a \mymid s) = \frac{1}{2}, \qquad \forall (s,a,h)\in \cS\times \cA\times [H], 
\end{align}
%
where $\mu$ has been defined in \eqref{finite-mu-assumption}. 
As it turns out, for any MDP $\mathcal{M}_\phi$, the occupancy distributions of the above batch dataset admit the following simple characterization: 
%
\begin{align}
     \frac{\mu(s)}{2} \leq  d^{\mathsf{b}, P^\phi}_h(s) \leq 2\mu(s), \qquad  \frac{\mu(s)}{4} \leq  d^{\mathsf{b}, P^\phi}_h(s,a) \leq \mu(s), \qquad \forall (s,a,h)\in\cS\times \cA\times [H]. 
    \label{eq:finite-lb-behavior-distribution}
\end{align}
%
In addition, we choose the following initial state distribution $\rho$
\begin{align}
    \rho(s) = 
    \begin{cases} 1, \quad &\text{if }s=0, \\
        0, &\text{if }s>0,
    \end{cases}
    %
    \label{eq:rho-defn-finite-LB}
\end{align}
which directly yields that the robust single-policy clipped concentrability coefficient $\Cstar$ and the quantity $C$ are connected as follows:
%
\begin{align}
    \Cstar = 4C. \label{eq:expression-Cstar-LB-finite}
\end{align}
%
The proof of the claims \eqref{eq:finite-lb-behavior-distribution} and \eqref{eq:expression-Cstar-LB-finite} are postponed to Appendix~\ref{proof:eq:finite-lb-behavior-distribution}.


\subsection{Key properties of the constructed MDPs}
\paragraph{Uncertainty set of the transition kernels.}
Let the uncertainty level be $\ror$. Specifically, for any $(s,a,h)\in \cS\times\cA\times [H]$, the perturbation of the transition kernel is restricted to the following uncertainty set
\begin{align}
    \unb^\ror(P^{\phi})\defn \otimes \; \unb^\ror (P^{\phi}_{h,s,a}),\qquad \unb^\ror(P_{h,s,a}^{\phi}) \defn \left\{ P_{h, s,a} \in \Delta (\cS): \mathsf{KL}\left(P_{h,s,a} \parallel P^{\phi}_{h,s,a}\right) \leq \ror \right\}.
\end{align}
With this in hand, for any $P^{\phi}_h(\cdot  \mymid s, a)$ and value function vector $V$, we denote the corresponding transition kernel vector in the worst case by
\begin{align}
    P^{\inf, \phi}_{h,s,a}(V) &\defn  \mathrm{argmin}_{\cP \in \unb^{\ror}(P^{\phi}_{h,s,a})}  \cP V \in [0,1]^{1\times S},
\end{align}
and its $s'$-th row by
\begin{equation}
   P^{\inf, \phi}_{h}(s'\mymid s,a, V) \defn \left[P^{\inf, \phi}_{h,s,a}(V)\right](s').
\end{equation}
In addition, for any $P^{\phi}_h(\cdot  \mymid s, a)$ in \eqref{eq:Ph-construction-lower-finite} or \eqref{eq:Ph-construction-lower-finite-h}, we define the limit of the perturbed transition kernel
\begin{align}\label{eq:finite-lw-def-p-q}
\underline{P}^{\phi}_{h}(s' \mymid s,a) &\defn \inf_{P_{h,s,a} \in \unb^{\ror}(P^{\phi}_{h,s,a})} P_h(s'  \mymid s,a),
\end{align}
and specially
\begin{align}\label{eq:finite-lw-p-q-perturb-inf}
\underline{p} &\defn \underline{P}^{\phi}_{h}(0 \mymid 0,\phi_h)  ,\quad \underline{q} = \underline{P}^{\phi}_{h}(0  \mymid 0, 1-\phi_h).
\end{align}
With these notations in mind, we introduce the following lemma which indicate some useful properties of the uncertainty set.
\begin{lemma}\label{lem:finite-lb-uncertainty-set}
When the uncertainty level $\ror$ obeys 
\begin{align}
\left(1- \frac{3}{\cq}\right)\log(H) \leq \ror \leq \left(1- \frac{2}{\cq}\right)\log(H),
\end{align} the perturbed transition kernels obey
\begin{align}\label{eq:finite-lw-upper-p-q}
   \underline{p}\geq \underline{q} \geq \frac{1}{\cq}.
\end{align}
\end{lemma}
\begin{proof}
See Appendix~\ref{proof:lem:finite-lb-uncertainty-set}.
\end{proof}




\paragraph{Value functions and optimal policies.}

We take a moment to see the corresponding value functions and  identify the optimal policies. To abuse the notation, for any MDP $\cM^\phi$, we denote $\pi^{\star,\phi} = \{\pi^{\star,\phi}_h\}_{h=1}^H$ as the optimal policy, and let $V_{h}^{\pi, \phi, \ror}$ (resp.~$V_{h}^{\star, \phi, \ror}$) represent the value function of policy $\pi$ (resp.~$\pi^{\star,\phi}$) at time step $h$. Moreover, for notational conciseness, we shall use the shorthand $V_{h}^{\pi, \phi} = V_{h}^{\pi, \phi, \ror}$ and $V_{h}^{\star, \phi} = V_{h}^{\star, \phi, \ror}$ when it is  clear from the context.

Armed with the notations, we introduce the following lemma which collects the properties concerning the value functions and optimal policies.
\begin{lemma}\label{lem:finite-lb-value}
For any $\phi\in\Phi$ and any policy $\pi$, defining 
\begin{align}
z_{\phi}^{\pi} \defn \underline{p}\pi_h(\phi_h\mymid 0) + \underline{q} \pi_h(1-\phi_h\mymid 0),\label{eq:finite-x-h}
\end{align}
it holds that
%
\begin{align}
    V_1^{\pi, \phi}(0) =  1 + z_{\phi}^{\pi} (H-1).
    \label{eq:finite-lemma-value-0-pi}
\end{align}
%
In addition,  for any $h\in[H]$,  the optimal policies and the optimal value functions obey
%
\begin{subequations}
    \label{eq:finite-lb-value-lemma}
\begin{align}
    \pi_h^{\star,\phi}(\phi \mymid 0) &= 1, \qquad V_h^{\star, \phi}(0) = H - h + 1, \qquad &\forall 1<h\leq H, \\
    \pi_h^{\star,\phi}(1 \mymid 0) &= 1, \qquad V_h^{\star, \phi}(1) = 0, \qquad &\forall h\in[H].
\end{align}
%
\end{subequations}
%
\end{lemma}
\begin{proof}
See Appendix~\ref{proof:lem:finite-lb-value}.
\end{proof}

\subsection{Establishing the minimax lower bound}
We are now ready to establish the sample complexity lower bound. With the choice of the initial distribution $\rho$ in \eqref{eq:rho-defn-finite-LB}, for any policy estimator $\widehat{\pi}$ computed based on the batch dataset, we plan to control the quantity
$$\big\langle \rho, V_1^{\star, \phi} - V_1^{\widehat{\pi}, \phi} \big\rangle = V_1^{\star, \phi}(0) - V_1^{\widehat{\pi}, \phi}(0).$$

\paragraph{Step 1: converting the goal to estimate $\phi$.}
Towards this, we make the following claim which shall be verified in Appendix~\ref{proof:finite-lower-diff-control}:
%
\begin{align}
    \big\langle \rho, V_1^{\star, \phi} - V_1^{\pi, \phi} \big\rangle  \geq 2\varepsilon \big(1-\pi_1(\phi\mymid 0)\big) \label{eq:finite-Value-0-recursive}
\end{align}
holds by choosing 
\begin{align}\label{eq:Delta-chosen}
    \Delta = \frac{\ror \varepsilon}{ 6H \left( e^{(H-1)/\lambda^\star} -1\right)},
\end{align}
where $\lambda^\star$ is some variable that obeys $\lambda^\star \in (0, \frac{12}{7c_1}]$.

Armed with this relation between policy $\pi$ and the performance gap, we are positioned to construct an estimation for $\phi$. We denote $\mathbb{P}_\phi$ as the probability distribution when the MDP is $\mathcal{M}_\phi$, for any $\phi \in \Phi$.


Suppose for the moment that a policy estimate $\widehat{\pi}$ achieves
%
\begin{align}
    \mathbb{P} \left\{\big\langle \rho, V_1^{\star, \phi} - V_1^{\widehat{\pi}, \phi} \big\rangle \leq \varepsilon\right\} \geq \frac{7}{8},
    \label{eq:assumption-theta-small-LB-finite}
\end{align}
%
then in view of \eqref{eq:finite-Value-0-recursive}, 
we necessarily have $\pi_1(\phi\mymid 0) \geq \frac{1}{2}$ with probability at least $\frac{7}{8}$.
%
% \begin{equation}
%     \mathbb{P}\left\{ \sum_{h=1}^H \big\| \widehat{\pi}_h(\cdot\mymid 0) - \pi_h^{\star, \phi}(\cdot\mymid 0) \big\|_1 < H/8 \right\} \geq \frac{3}{4}.
% \end{equation}

% Following the pipeline in Step 1 in \cite[Appendix~C.2.2]{li2022settling}, 
With this in mind, we are motivated to construct the following estimate $\widehat{\phi}$ for $\phi\in \Phi$: 
\begin{align}
    \widehat{\phi}=\arg\max_{a} \, \widehat{\pi}(a\mymid 0),
    \label{eq:defn-theta-hat-inf-LB}
\end{align}
which obeys
\begin{align}
    \mathbb{P}_{\phi}\big( \widehat{\phi} = \phi \big) 
    \geq \mathbb{P}_{\phi}\big\{ \widehat{\pi}_1(\phi \mymid 0) > 1/2 \big\} \geq \frac{7}{8}. 
    \label{eq:P-theta-accuracy-inf}
\end{align}
%
In what follows, we would like to show \eqref{eq:P-theta-accuracy-inf} cannot happen without enough samples, which would in turn contradict \eqref{eq:finite-Value-0-recursive}. 

 

\paragraph{Step 2: probability of error in testing two hypotheses.}
Towards this, we shall convert the estimation of $\phi$ into differentiating two hypotheses $\phi = 0$ and $\phi=1$. 

We denote $\mathbb{P}_\phi$ as the probability distribution when the MDP is $\mathcal{M}_\phi$, for any $\phi \in \Phi$. Then, we will study the minimax probability of error defined as follows:
%
\begin{equation}
    p_{\mathrm{e}} \coloneqq \inf_{\phi}\max \big\{ \mathbb{P}_{0}(\phi \neq 0), \mathbb{P}_{1}(\phi \neq 1) \big\} , \label{eq:error-prob-two-hypotheses-finite-LB}
\end{equation}
%
where the infimum is taken over all possible tests constructed based on the batch dataset available.

Let $\mu^{\mathsf{b},\phi}$ (resp.~$\mu^{\mathsf{b},\phi}_h(s_h)$) represent the distribution of a sample trajectory $\{s_h, a_h\}_{h=1}^H$ (resp.~a sample $(a_h,s_{h+1})$ conditional on $s_h$) for the MDP $\mathcal{M}_\phi$. Recalling that the $K$ trajectories in the batch dataset are independently generated, one has
\begin{align}
p_{\mathrm{e}} & \overset{\mathrm{(i)}}{\geq}\frac{1}{4}\exp\Big(- K\mathsf{KL} \big(\mu^{\mathsf{b},0}\parallel \mu^{\mathsf{b},1} \big)\Big)\nonumber\\
    & = \frac{1}{4}\exp\bigg\{-\frac{1}{2}K\mu(0)\Big(\mathsf{KL}\big(P_{1}^0(\cdot\mymid0,0)\parallel P_{1}^1(\cdot\mymid0,0)\big)+\mathsf{KL}\big(P_{1}^0(\cdot\mymid0,1)\parallel P_{1}^1(\cdot\mymid0,1)\big)\Big)\bigg\}. 
    \label{eq:finite-remainder-KL}
\end{align}
where (i) results from \citet[Theorem~2.2]{tsybakov2009introduction} and  the additivity property of the KL divergence (cf.~\citet[Page~85]{tsybakov2009introduction}). Here, (ii) arises from invoking the chain rule of the KL divergence \citep[Lemma 5.2.8]{duchi2018introductory} and the Markovian nature of the sample trajectories to obtain
%
\begin{align*}
\mathsf{KL}\big(\mu^{\mathsf{b},0}\parallel\mu^{\mathsf{b},1}\big) & =\sum_{h=1}^{H}\mathop{\mathbb{E}}\limits _{s_{h}\sim d^{\mathsf{b}, P^\phi}_{h}}\left[\mathsf{KL}\big(\mu_{h}^{\mathsf{b},0}(s_{h})\parallel\mu_{h}^{\mathsf{b},1}(s_{h})\big)\right] =\sum_{h=1}^H\sum_{a\in\{0,1\}}  d^{\mathsf{b}, P^\phi}_{h}(0,a)\mathsf{KL}\left(P_{h}^{0}(\cdot\mymid0,a)\parallel P_{h}^{1}(\cdot\mymid0,a)\right)  \\
    &= \frac{1}{2}\mu(0)\sum_{a}\mathsf{KL}\big(P_{1}^{0}(\cdot\mymid0,a)\parallel P_{1}^{1}(\cdot\mymid0,a)\big),
\end{align*}
where the last two inequalities hold by \eqref{eq:finite-lb-behavior-distribution} and the fact that $P_{h}^{0}(\cdot\mymid s,a), P_{h}^{1}(\cdot\mymid s,a)$ only differ when $h=1$ and $s=0$.

% Applying the proof pipeline in Step 2 in \cite[Appendix~C.2.2]{li2022settling}, combined with the property of $\Phi$ in \eqref{eq:property-Theta}, using Fano's inequality (cf.~\citep[Corollary 2.6]{tsybakov2009introduction}) and properties of KL divergence, we arrive at
% \begin{align}
%     p_{\mathrm{e}} \geq \frac{1}{2}- \frac{4K \mu(0)}{H} \max_{\phi,\widetilde{\phi}\in \Phi, \, \phi\neq \widetilde{\phi}} \, \sum_{h=1}^H     \left[ \mathsf{KL}\big( P_{h}^{\phi}(\cdot \mymid 0, 0) \parallel  P_{h}^{\widetilde{\phi}}(\cdot \mymid 0, 0)  \big) + \mathsf{KL}\big( P_{h}^{\phi}(\cdot \mymid 0, 1) \parallel  P_{h}^{\widetilde{\phi}}(\cdot \mymid 0, 1)  \big)  \right] .
%     \label{eq:finite-remainder-KL}
% \end{align}

% So now we turn to control the KL divergence terms in \eqref{eq:finite-remainder-KL}. In the first case when $\phi_h = \widetilde{\phi}_h$, it is easily verified that
% %
% \begin{align}
%    \mathsf{KL}\big( P_{h}^{\phi}(\cdot \mymid 0, 0) \parallel  P_{h}^{\widetilde{\phi}}(\cdot \mymid 0, 0)  \big) + \mathsf{KL}\big( P_{h}^{\phi}(\cdot \mymid 0, 1) \parallel  P_{h}^{\widetilde{\phi}}(\cdot \mymid 0, 1)  \big)  = 0. \label{eq:finite-KL-bounded-0}
% \end{align}
% %
% Next, we consider the case that $\phi_h \neq \widetilde{\phi}_h$. Without loss of generality, let $\phi_h = 0$ and $\widetilde{\phi}_h = 1$.
% Invoking the expression
% %
% \begin{align*}
%     P_h^{\phi}(0 \mymid 0, 0)  &= P_h^{\phi_h}(\phi \mymid 0, 0) = \left(1 -\frac{1}{CS}\right)p + \frac{1}{CS},\\
%     P_h^{\widetilde{\phi}}(0 \mymid 0, 0) &= P_h^{\widetilde{\phi}}\big(1-\widetilde{\phi}_h \mymid 0, 0\big) = \left(1 -\frac{1}{CS}\right)q + \frac{1}{CS}.
% \end{align*}
%

So now we turn to control the KL divergence terms in \eqref{eq:finite-remainder-KL}.
Given $p\geq q \geq 1/2$, applying Lemma~\ref{lem:KL-key-result} yields
%
\begin{align}
\mathsf{KL}\big(P_1^{0}(0 \mymid 0, 0)\parallel P_1^{1}(0 \mymid 0, 0)\big) & =\mathsf{KL}\left(p\parallel q \right) \frac{(p-q)^2}{(1-p)p}  \overset{\mathrm{(i)}}{\leq} \frac{\Delta^2}{p(1-p)} \notag\\
    & \overset{\mathrm{(ii)}}{=} \frac{ \ror^2 \varepsilon^2}{36H^2 \left( e^{(H-1)/\lambda^\star} -1\right)^2 p(1-p)} \notag \\
    & \overset{\mathrm{(iii)}}{\leq} \frac{ \ror\varepsilon^2}{ 9H^2  e^{2(H-1)/\lambda^\star} \cdot e^{-12(H-1)/7\lambda^\star}} \notag \\
    & \overset{\mathrm{(iv)}}{\leq} \frac{ \ror^2 \varepsilon^2}{  9H^2 e^{2(H-1)/7\lambda^\star}} \leq  \frac{ \ror^2 \varepsilon^2}{ 9H^2  e^{c_1(H-1)/6}},
    \label{eq:finite-KL-bounded}
\end{align}
%
where (i) follows from the definition \eqref{eq:finite-p-q-def} of $(p, q)$, (ii) holds by the fact in \eqref{eq:Delta-chosen}, (iii) and (iv) can be verified by letting $\left( e^{(H-1)/\lambda^\star} -1\right)^2 \geq \frac{1}{2} e^{2(H-1)/\lambda^\star}$ and \eqref{eq:finite-lower-check-lambda-star}.
It can be shown that $\mathsf{KL}\big(P_1^{0}(0 \mymid 0, 1)\parallel P_1^{1}(0 \mymid 0, 1)\big)$ 
can be upper bounded in the same way. 
Substituting \eqref{eq:finite-KL-bounded} back into \eqref{eq:finite-remainder-KL} 
demonstrate that: if the sample size does not exceed
\begin{align}\label{eq:finite-sample-N-condition}
    KH \leq \frac{9H^2 e^{c_1(H-1)/6} H^3CS \log 2}{ \ror^2 \varepsilon^2},
\end{align}
then one necessarily has
\begin{align}
    p_{\mathrm{e}} \geq \frac{1}{4}\exp\bigg\{-\frac{1}{2}K\mu(0) \frac{ 2\ror^2 \varepsilon^2}{  9H^2  e^{c_1(H-1)/6} }  \bigg\} = \frac{1}{4}\exp\bigg\{\frac{-K \ror^2 \varepsilon^2}{ 9CS H^2 e^{c_1(H-1)/6} } \bigg\}  \geq \frac{1}{8}. \label{eq:pe-LB-13579-inf}
\end{align}

\paragraph{Step 3: putting all this together.} 
%
Finally, suppose that there exists an estimator $\widehat{\pi}$ such that
%
\[
    \mathbb{P}_0 \big\{  \big\langle \rho, V_1^{\star, 0} - V_1^{\widehat{\pi}, 0} \big\rangle > \varepsilon  \big\} < \frac{1}{8}
    \qquad \text{and} \qquad
    \mathbb{P}_1 \big\{  \big\langle \rho, V_1^{\star,1} - V_1^{\widehat{\pi},1} \big\rangle > \varepsilon  \big\} < \frac{1}{8}.
\]
%
Then in view of the analysis in Step 1, the estimator $\widehat{\phi}$ defined in \eqref{eq:defn-theta-hat-inf-LB} must satisfy
%
\[
    \mathbb{P}_0\big(\widehat{\phi} \neq 0\big) < \frac{1}{8} 
    \qquad \text{and} \qquad
    \mathbb{P}_1\big(\widehat{\phi} \neq 1\big) < \frac{1}{8}. 
\]
%
This, however, cannot possibly happen under the sample size condition \eqref{eq:finite-sample-N-condition}; otherwise it is contradictory to the result in \eqref{eq:pe-LB-13579-inf}. 

\subsubsection{Proof of Lemma~\ref{lem:finite-lb-uncertainty-set}}\label{proof:lem:finite-lb-uncertainty-set}

Note that $\underline{p} \geq \underline{q}$ can be easily verified since $p>q$, which indicates that the first assertion is true. So we will focus on the second assertion in \eqref{eq:finite-lw-upper-p-q}. Towards this, let $\ror'$ be the following term
\begin{align}
    \ror' & \defn \mathsf{KL}\left(\mathsf{Ber}\left(\frac{1}{\cq}\right) \parallel \mathsf{Ber}(q)\right) = \frac{1}{\cq}\log\frac{\frac{1}{\cq}}{q} + \left(1- \frac{1}{\cq}\right)\log\frac{\left(1- \frac{1}{\cq}\right)}{1-q} \notag \\
    & \overset{\mathrm{(i)}}{=} \left(\frac{1}{\cq}\right)\log\left(\frac{1}{\cq}\right) - \left(\frac{1}{\cq}\right) \log(q) + \left(1- \frac{1}{\cq}\right)\log(H) - \left(1- \frac{1}{\cq}\right)\log(c_1)  + \left(1- \frac{1}{\cq}\right)\log\left(1- \frac{1}{\cq}\right),
    \end{align}
where (i) holds by the definition of $q$ in \eqref{eq:finite-p-q-def}.
Observing $\frac{1}{2} \leq q = 1-\frac{c_1}{H} \leq 1 $, when $H\geq c_2 c_1 \cq$ with $c_2$ large enough, basic calculus gives
\begin{align}\label{eq:finite-lower-ror-bounded}
    \left(1- \frac{2}{\cq}\right)\log(H) \leq \ror' \leq \left(1- \frac{1}{\cq}\right)\log(H).
\end{align}
To continue, choosing $$ \left(1- \frac{3}{\cq}\right)\log(H) \leq \ror \leq \left(1- \frac{2}{\cq}\right)\log(H) \leq \ror',$$ we have for any $[q',1-q']\in \unb^\ror([q,1-q])$,
\begin{align}
    \mathsf{KL}\left(\mathsf{Ber}\left(q'\right) \parallel \mathsf{Ber}(q)\right) \leq \mathsf{KL}\left(\mathsf{Ber}\left(\frac{1}{\cq}\right) \parallel \mathsf{Ber}(q)\right),
\end{align}
which directly indicates 
\begin{align}
    \underline{q} = \inf_{[q',1-q'] \in \unb^\ror([q,1-q])} q' \geq \frac{1}{\cq}.
\end{align}

% Then, to study $\underline{q}$ based on the uncertainty level $\ror$. given $\mathsf{KL}\big(\mathsf{Ber}(\underline{q} \parallel \mathsf{Ber}(q_0)\big) \leq \ror(\Phi)$, we have the following relation can't happen
% \begin{align}
%     2\left\|\mathsf{Ber}(\underline{q}) - \mathsf{Ber}(q)\right\|_{\mathsf{TV}}^2 = 8|\underline{q}- q_0|^2 \geq \ror(\Phi) \geq \mathsf{KL}\big(\mathsf{Ber}(\underline{q}) \parallel \mathsf{Ber}(q)\big).
% \end{align}
% So 
% \begin{align}
%     \underline{q} \geq q_0 - \sqrt{\frac{\ror(\Phi)}{8}} \geq 1 - e^{-c_1H} - \sqrt{\frac{\ror(\Phi)}{8}} \geq 1- 2e^{-c_1 H}
% \end{align}
% when the uncertainty set $\ror(\Phi)$ obeys
% \begin{equation}
%     \sqrt{\frac{\ror(\Phi)}{8}} \leq e^{-c_1 H}.
% \end{equation}
% So $\ror(\Phi) \leq 8 e^{-2c_1H}$.


\subsubsection{Proof of Lemma~\ref{lem:finite-lb-value}}\label{proof:lem:finite-lb-value}

% To start with, with abuse of notation, we introduce
% \begin{align}
%     P_{h,s,a}^{\phi} \defn P^{\phi}_h(\cdot \mymid s,a) \in [0,1]^{1\times S}.
% \end{align}


For  any policy $\pi$, we observe that the value function of the state $1$ at any time step $h\in[H]$ obeys
\begin{align}
    V_h^{\pi,\phi}(1) &= \mathbb{E}_{a\in\pi_h(\cdot \mymid 1)}\left[r_h(1,a) + \inf_{ \cP \in \unb^{\sigma}(P^{\phi}_{h,s,a})}  \cP  V_{h+1}^{\pi,\phi}\right] = 0 + V_{h+1}^{\pi,\phi}(1),
\end{align}
which recursively yields the following fact
\begin{align}
    V_h^{\star,\phi}(1) = V_h^{\pi,\phi}(1) = 0,\qquad \forall h\in[H]. \label{eq:finite-s-1-upper-value}
\end{align}

% \paragraph{Step 1: characterizing the facts about state $1$}
% \begin{align}
%      V_h^{\pi,\phi}(1) &= \mathbb{E}_{a\in\pi_h(\cdot \mymid 1)}\left[r_h(1,a) + \inf_{P\in \cB\big(P_{h,1,a}^{\phi}, \ror\big)}\; P  V_{h+1}^{\pi,\phi}\right] \notag \\
%      & = \pi_h(0 \mymid 1) \left( \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) \right)+ \pi_h(1\mymid 1)\left[ P^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(1) + \left(1-P^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right)\right) V_{h+1}^{\pi,\phi}(0)\right] \label{eq:finite-s-1-equal-value} \\
%       & \leq \pi_h(0 \mymid 1) \left( \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) \right)+ \pi_h(1\mymid 1)\left[ P^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(1) + \left(1-\underline{P}^{\phi}_{h}\left(1 \mymid 1,1\right)\right) V_{h+1}^{\pi,\phi}(0)\right] \notag \\
%      & \overset{\mathrm{(i)}}{\leq} \pi_h(0 \mymid 1) \left( \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) \right)+ \pi_h(1\mymid 1)\left[ P^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(1) + \frac{c_2}{H} (H-h)\right] \notag\\
%      & \overset{\mathrm{(ii)}}{\leq} \pi_h(0 \mymid 1) \left( \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) \right)+ \pi_h(1\mymid 1)\Big[ \frac{1}{2} + PP^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(1)\Big] \notag\\
%      & = \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) - \left(1 - P^{\inf, \phi}_{h}\left(1 \mymid 1,1, V_{h+1}^{\pi,\phi}\right)\right) \pi_h(1\mymid 1) V_{h+1}^{\pi,\phi}(1), \label{eq:finite-s-1-upper-value}
% \end{align}
% where (i) holds by applying \eqref{eq:finite-lw-upper-p-q} and the trivial fact $0\leq V_{h}^{\pi,\phi}\leq H-h+1$ for any policy $\pi$ and time step $h\in[H]$, (ii) arises from $\frac{c_2}{H} (H-h)\leq \frac{1}{2}$ when $c_2$ is small enough. The above results directly leads to several facts:
% \begin{itemize}
%     \item Choosing the policy $\pi$ as $\pi_h(0\mymid 1) =1$, in view of \eqref{eq:finite-s-1-equal-value}, we recursively arrive at
%     \begin{align}
%         V_h^{\pi,\phi}(1) = \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) =\cdots = \frac{1}{2}(H-h+1).
%     \end{align}

%     \item For any policy $\pi$, applying \eqref{eq:finite-s-1-upper-value} recursively shows that
%     \begin{align}
%          V_h^{\pi,\phi}(1) \leq \frac{1}{2} + V_{h+1}^{\pi,\phi}(1) \leq \cdots \leq \frac{1}{2}(H-h+1).
%     \end{align}
% \end{itemize}
% Summing up the results in above two cases indicates that, in state $1$, the optimal policies and optimal value functions obey
% \begin{align}\label{eq:finite-optimal-value-1}
%     \pi_h^\star(0 \mymid 1) = 1, \qquad V_h^{\star, \phi}(1) = \frac{1}{2}(H-h+1), \qquad \forall h\in[H].
% \end{align}

% \paragraph{Step 2: characterizing the facts about state $0$}
% \begin{align}
%     V_h^{\pi,\phi}(0) &= \mathbb{E}_{a\in\pi_h(\cdot \mymid 0)}\left[1 + \inf_{P\in \cB\big(P_{h,0,a}^{\phi}, \ror\big)}\; P  V_{h+1}^{\pi,\phi}\right] \notag \\
%     & = 1 + \pi_h(\phi_h \mymid 0)\Big[ P^{\inf, \phi}_{h}\left(0 \mymid 0, \phi_h, V_h^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{h}\left(0 \mymid 0, \phi_h,V_h^{\pi,\phi}\right) \right) V_{h+1}^{\pi,\phi}(1)\Big] \notag\\
%     &\quad + \pi_h(1-\phi_h \mymid 0)\Big[ P^{\inf, \phi}_{h}\left(0 \mymid 0, 1- \phi_h, V_h^{\pi,\phi}\right)V_{h+1}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{h}\left(0 \mymid 0, 1-\phi_h,V_h^{\pi,\phi}\right) \right) V_{h+1}^{\pi,\phi}(1)\Big] \label{eq:finite-value-0-equal} \\
%     & \geq 1 + \left(\pi_h(\phi_h \mymid 0) \underline{P}^{\phi}_{h}(0 \mymid 0, \phi_h) + \pi_h(1-\phi_h \mymid 0) \underline{P}^{\phi}_{h}(0 \mymid 0, 1-\phi_h)  \right) V_{h+1}^{\pi,\phi}(0) \notag\\
%     & \overset{\mathrm{(i)}}{\geq} 1 + \overline{q} V_{h+1}^{\pi,\phi}(0)  \geq \sum_{i=0}^{H-h} (\overline{q})^i \overset{\mathrm{(ii)}}{\geq} \sum_{i=0}^{H-h}\left(1- \frac{c_2}{H}\right)^i \overset{\mathrm{(iii)}}{\geq} \frac{2}{3}(H+1-h) . \label{eq:finite-value-0-lower-bounded}
% \end{align}
% where (i) and (ii) hold by the fact $\overline{p} > \overline{q} \geq 1-\frac{c_2}{H}$ (see Lemma~\ref{lem:finite-lb-uncertainty-set}), (iii) arises from
% \begin{align}\label{eq:finite-c2-contraction-bounded}
%     \left(1- \frac{c_2}{H}\right)^{H-h+1} \geq \left(1- \frac{c_2}{H}\right)^{H} \geq \exp\left(H 
% \log\left(1- \frac{c_2}{H}\right)\right) \geq e^{-2c_2} \geq \frac{2}{3}
% \end{align}
% where the last two inequalities follows from the fact $\log(1+x) \geq 2x$ when $x\in[-1/2,0]$ and $c_2\in(0,1/2]$ can be small enough. Combining the results in \eqref{eq:finite-value-0-lower-bounded} and \eqref{eq:finite-optimal-value-1}, the following fact
% \begin{equation}
%     V_h^{\star, \phi}(0) \geq V_h^{\pi, \phi}(0) \geq \frac{2}{3}(H+1-h) > V_h^{\star, \phi}(1)
% \label{eq:finite-value-0-lower-bounded}
% \end{equation}
% holds for any policy $\pi$ and $h\in[H]$. With this in mind, next, we introduce a important fact which will be used later: for any value function vector $0\leq \|V\|_\infty \leq H$, we have
% \begin{align}
%     P^{\inf, \phi}_{h}\left(0 \mymid 0, a, V \right) = \underline{P}^{\phi}_{h}(0 \mymid 0,a),\qquad \forall a\in\{0,1\}, \label{eq:finite-lower-P-pro1}
% \end{align}
% which follows from the fact that $V_h^{\pi, \phi}(0)\geq V_h^{\pi, \phi}(1)$ for any $\pi$, leading to that the the worst case is under the transition kernel with the smallest probability moving to state $0$.

% To continue, plugging in \eqref{eq:finite-value-0-equal}, we further investigate the value at state $0$ as follows
% \begin{align}
%     V_h^{\pi,\phi}(0) 
%     & = 1 + \pi_h(\phi_h \mymid 0)\Big[ P^{\inf, \phi}_{h}\left(0 \mymid 0, \phi_h, V_h^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{h}\left(0 \mymid 0, \phi_h,V_h^{\pi,\phi}\right) \right) V_{h+1}^{\pi,\phi}(1)\Big] \notag\\
%     &\quad + \pi_h(1-\phi_h \mymid 0)\Big[ P^{\inf, \phi}_{h}\left(0 \mymid 0, 1- \phi_h, V_h^{\pi,\phi}\right)V_{h+1}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{h}\left(0 \mymid 0, 1-\phi_h,V_h^{\pi,\phi}\right) \right) V_{h+1}^{\pi,\phi}(1)\Big] \notag \\
%     & \overset{\mathrm{(i)}}{=} 1 + \pi_h(\phi_h \mymid 0)\Big[ \underline{p} V_{h+1}^{\pi,\phi}(0) + \left(1- \underline{p}\right) V_{h+1}^{\pi,\phi}(1)\Big] + \pi_h(1-\phi_h \mymid 0)\Big[ \underline{q} V_{h+1}^{\pi,\phi}(0) + \left(1-\underline{q} \right) V_{h+1}^{\pi,\phi}(1)\Big] \notag\\
%     & \overset{\mathrm{(ii)}}{=} 1 + V_{h+1}^{\pi,\phi}(1) + z_h^{\pi,\phi}  \left[V_{h+1}^{\pi,\phi}(0) - V_{h+1}^{\pi,\phi}(1) \right] 
% \end{align}
% where (i) follows from applying \eqref{eq:finite-lower-P-pro1} and \eqref{eq:finite-lw-p-q-perturb-inf}, and (ii) holds by choosing
% \begin{align}
% z_h^{\pi,\phi} \defn \underline{p}\pi_h(\phi_h\mymid 0) + \underline{q} \pi_h(1-\phi_h\mymid 0).
% \end{align}
Similarly, for any policy $\pi$, we observe that the value function of the state $0$ at time step $h>1$ satisfies
\begin{align}
    V_h^{\pi,\phi}(0) &= \mathbb{E}_{a\in\pi_h(\cdot \mymid 0)}\left[1 + \inf_{P\in \cB\big(P_{h,0,a}^{\phi}, \ror\big)}\; P  V_{h+1}^{\pi,\phi}\right] = 1 + V_{h+1}^{\pi,\phi}(0),
\end{align}
which recursively gives
\begin{align}
    V_h^{\star,\phi}(0) = V_h^{\pi,\phi}(0) = H-h+1, \qquad \forall h\in[H]. \label{eq:finite-s-0-h-upper-value}
\end{align}

Note that $V_h^{\pi,\phi}(0) > V_h^{\pi,\phi}(1)$ for all $1<h\leq H$, which is implied by \eqref{eq:finite-s-1-upper-value} and \eqref{eq:finite-s-0-h-upper-value}.
As a result, at time step $h=1$,
\begin{align}
    V_1^{\pi,\phi}(0) &= \mathbb{E}_{a\in\pi_1(\cdot \mymid 0)}\left[1 + \inf_{P\in \cB\big(P_{1,0,a}^{\phi}, \ror\big)}\; P  V_{2}^{\pi,\phi}\right] \notag \\
    & = 1 + \pi_1(\phi \mymid 0)\Big[ P^{\inf, \phi}_{1}\left(0 \mymid 0, \phi, V_2^{\pi,\phi}\right) V_{2}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{1}\left(0 \mymid 0, \phi, V_{2}^{\pi,\phi}\right) \right) V_{2}^{\pi,\phi}(1)\Big] \notag\\
    &\quad + \pi_1(1-\phi \mymid 0)\Big[ P^{\inf, \phi}_{1}\left(0 \mymid 0, 1- \phi, V_2^{\pi,\phi}\right)V_{2}^{\pi,\phi}(0) + \left(1-P^{\inf, \phi}_{1}\left(0 \mymid 0, 1-\phi,V_2^{\pi,\phi}\right) \right) V_{2}^{\pi,\phi}(1)\Big] \notag \\
    & \overset{\mathrm{(i)}}{=} 1 + \pi_1(\phi \mymid 0)\Big[ \underline{p} V_{2}^{\pi,\phi}(0) + \left(1- \underline{p}\right) V_{2}^{\pi,\phi}(1)\Big] + \pi_1(1-\phi \mymid 0)\Big[ \underline{q} V_{2}^{\pi,\phi}(0) + \left(1-\underline{q} \right) V_{2}^{\pi,\phi}(1)\Big] \notag\\
    & \overset{\mathrm{(ii)}}{=} 1 + V_{2}^{\pi,\phi}(1) + z_{\phi}^{\pi}  \left[V_{2}^{\pi,\phi}(0) - V_{2}^{\pi,\phi}(1) \right] \notag\\
    & = 1 + z_{\phi}^{\pi} V_{2}^{\pi,\phi}(0)
\end{align}
where (i) follows from \eqref{eq:finite-lw-p-q-perturb-inf}, (ii) holds by choosing
\begin{align}\label{eq:defination-z-phi-pi}
z_{\phi}^{\pi} \defn \underline{p}\pi_1(\phi\mymid 0) + \underline{q} \pi_h(1-\phi\mymid 0),
\end{align}
and the last inequality holds by \eqref{eq:finite-s-1-upper-value}


Therefore, we directly arrive at
\begin{align}
    V_1^{\star,\phi}(0) = 1 + z_{\phi}^{\star} V_{2}^{\star,\phi}(0) = 1 + z_{\phi}^{\star} (H-1).
\end{align} 
Observing that the function $(H-1)z$ is increasing in $z$ and that $z_{\phi}^{\star}$ is increasing in $\pi_1(\phi \mymid 0)$ (since $p\geq q$ leads to $\underline{p}\geq \underline{q}$).
As a result, we can conclude that the optimal policy in state $0$ obeys
%
\begin{equation}
    \pi_1^{\star,\phi}(\phi \mymid 0) = 1,\qquad \text{for all } h\in[H]. \label{eq:finite-lb-optimal-policy}
\end{equation}

\subsubsection{Proof of auxiliary facts}\label{proof:eq:finite-lb-behavior-distribution}


\paragraph{Proof of claim \eqref{eq:finite-lb-behavior-distribution}.}
With the initial distribution and policy defined in \eqref{eq:lower-dataset-assumption}, we have
\begin{align}
     d^{\mathsf{b}, P^\phi}_1(s) = \rhob (s) = \mu(s).
\end{align}
In addition, the occupancy distributions in the next step $h=2$ obey
\begin{align}
    d^{\mathsf{b}, P^\phi}_2(0) &= \mathbb{P}\{s_2 = 0 \mymid s_1\sim d^{\mathsf{b}, P^\phi}_1 ; \pib\}  = \mu(0)\left[\pib_1(\phi \mymid 0)p + \pib_1(1-\phi \mymid 0)q \right] = \frac{(p+q)\mu(0)}{2},
    \end{align}
    and
    \begin{align}
     d^{\mathsf{b}, P^\phi}_2(1) &= \mathbb{P}\{s_2 = 1 \mymid s_1\sim  d^{\mathsf{b}, P^\phi}_1 ; \pib\} \notag \\
    &= \mu(0)\left[\pib_1(\phi \mymid 0)(1-p) + \pib_1(1-\phi \mymid 0)(1-q) \right] + \mu(1) = \mu(1) + \frac{(2-p-q)\mu(0)}{2}.
\end{align}
Recalling the assumption in \eqref{eq:lower-C-assumption} and \eqref{eq:lower-p-q-assumption}, we arrive at
\begin{align}
   \frac{\mu(0)}{2} \leq  d^{\mathsf{b}, P^\phi}_2(0) \leq \mu(0), \qquad \mu(1)\leq  d^{\mathsf{b}, P^\phi}_2(1) \leq 2\mu(1).
\end{align}
Finally, from the definitions of $P_h^\phi(\cdot \mymid s,a)$ in \eqref{eq:Ph-construction-lower-finite-h} and the Markov property, we arrive at for any $(h,s)\in [H] \times \cS$,
\begin{align}
   \frac{\mu(s)}{2} \leq  d^{\mathsf{b}, P^\phi}_h(s) \leq 2\mu(s),
\end{align}
which directly leads to
\begin{align}
    \frac{\mu(s)}{4} \leq  d^{\mathsf{b}, P^\phi}_h(s,a) = \pib_1(a\mymid s) d^{\mathsf{b}, P^\phi}_h(s) \leq \mu(s).
\end{align}

\paragraph{Proof of claim \eqref{eq:expression-Cstar-LB-finite}.}
Recalling $\pi_h^{\star,\phi}(\phi \mymid 0) =1$ for all $ h\in[H]$ in Lemma~\ref{lem:finite-lb-value} and $\rho(0) =1$, for any $P \sim \unb(P^\phi)$, we have
\begin{align}
    d_2^{\star, P}(0, \phi) &= d_2^{\star, P}(0)\pi_h^{\star,\phi}(\phi \mymid 0) = d_2^{\star, P}(0) = \mathbb{P}_{s_2 \sim P\left(\cdot \mymid s_1, \pi_1^{\star,\phi}(s_1) \right)}\{s_2 =0 \mymid s_1 \sim \rho ; \pi^{\star,\phi}\} \notag \\
    & = P_1(0 \mymid 0, \phi) = \underline{p} \geq \frac{1}{3}.
\end{align}
Then due to the Markov property and $P^\phi_h(0 \mymid 0, \phi) = 1$, we have
\begin{align}
    d_h^{\star, P}(0, \phi) = d_2^{\star, P}(0, \phi) \geq \frac{1}{3}.
\end{align}

Then invoking the definition of $\Cstar$ in \eqref{eq:concentrate-finite} yields
\begin{align}
    \max_{(s, a, P) \in \mathcal{S} \times \cA \times \unb^{\ror}(P^{\phi})} \frac{\min\big\{d_2^{\star,P}(s, a ), \frac{1}{S}\big\}}{ d^{\mathsf{b}, P^\phi}_2(s, a )}  &= \max_{P \in \unb^{\ror}(P^{\phi})} \frac{d_2^{\star,P}(0,\phi)}{d^{\mathsf{b}, P^\phi}_2(0, \phi )}  \leq \frac{4}{S\mu(0)} = 4C, \notag \\
    \max_{(s, a,  P) \in \mathcal{S} \times \cA \times \unb^{\ror}(P^{\phi})} \frac{\min\big\{d_1^{\star,P}(s, a ), \frac{1}{S}\big\}}{ d^{\mathsf{b}, P^\phi}_1(s, a )}  &= \max_{P \in \unb^{\ror}(P^{\phi})} \frac{d_1^{\star,P}(0,\phi)}{d^{\mathsf{b}, P^\phi}_1(0, \phi )}  \leq \frac{4}{S\mu(0)} = 4C, \notag\\
    \max_{(h,s, a, P) \in [H] \setminus\{1,2\} \times \mathcal{S} \times \cA \times \unb^{\ror}(P^{\phi})} \frac{\min\big\{d_h^{\star,P}(s, a ), \frac{1}{S}\big\}}{ d^{\mathsf{b}, P^\phi}_h(s, a )}  &= \max_{(h,P) \in [H] \setminus\{1,2\} \times  \unb^{\ror}(P^{\phi})} \frac{d_h^{\star,P}(0,\phi)}{d^{\mathsf{b}, P^\phi}_h(0, \phi )}  \leq \frac{4}{S\mu(0)} = 4C,
\end{align}
when $S \geq 3$.
So finally we arrive at
\begin{align}
    \Cstar = 4C.
\end{align}

\subsubsection{Proof of the essential claim \eqref{eq:finite-Value-0-recursive}.}\label{proof:finite-lower-diff-control}
% \paragraph{Step 1: expressing out the term of interest.}

% \begin{align}
%     \big\langle \rho, V_h^{\star, \phi} - V_h^{\pi, \phi} \big\rangle &= V_h^{\star, \phi}(0) - V_h^{\pi, \phi}(0) \notag \\
%     &= V_{h+1}^{\star,\phi}(1) + \underline{p}  \left[V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\star,\phi}(1) \right] - \left( V_{h+1}^{\pi,\phi}(1) + z_h^{\pi,\phi}  \left[V_{h+1}^{\pi,\phi}(0) - V_{h+1}^{\pi,\phi}(1) \right] \right) \notag \\
%     & =  z_h^{\pi,\phi} \left(V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\pi,\phi}(0)\right) + \left(\underline{p} - z_h^{\pi,\phi}\right)V_{h+1}^{\star,\phi}(0)  + \left(1- \underline{p}\right) V_{h+1}^{\star,\phi}(1) - \left(1- z_h^{\pi,\phi}\right) V_{h+1}^{\pi,\phi}(1)\notag \\
%     & \overset{\mathrm{(i)}}{\geq}  z_h^{\pi,\phi} \left(V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\pi,\phi}(0)\right) + \left(\underline{p} - z_h^{\pi,\phi}\right)V_{h+1}^{\star,\phi}(0)  + \left(1- \underline{p}\right) V_{h+1}^{\star,\phi}(1) - \left(1- z_h^{\pi,\phi}\right) V_{h+1}^{\star,\phi}(1)\notag \\
%     & = z_h^{\pi,\phi} \left(V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\pi,\phi}(0)\right) + \left(\underline{p} - z_h^{\pi,\phi}\right) \left(V_{h+1}^{\star,\phi}(0)  -V_{h+1}^{\star,\phi}(1) \right) \notag \\
%     & \overset{\mathrm{(ii)}}{\geq} \underline{q} \left(V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\pi,\phi}(0)\right) + \frac{1}{2}\left(\underline{p} - \underline{q}\right)\big\|\pi_{h}^{\star,\phi}(\cdot\mymid 0)-\pi_{h}(\cdot\mymid 0)\big\|_{1}\left(V_{h+1}^{\star,\phi}(0)  -V_{h+1}^{\star,\phi}(1) \right) \notag\\
%     & \geq \underline{q} \left(V_{h+1}^{\star,\phi}(0) - V_{h+1}^{\pi,\phi}(0)\right) + \frac{1}{12}\left(\underline{p} - \underline{q}\right)\big\|\pi_{h}^{\star,\phi}(\cdot\mymid 0)-\pi_{h}(\cdot\mymid 0)\big\|_{1}\left(H-h+1 \right) \label{eq:finite-lower-diff}
% \end{align}
% where (i) holds by $ V_{h+1}^{\pi,\phi}(1) \leq V_{h+1}^{\star,\phi}(1)$, (ii) follows from \eqref{eq:finite-x-h} implies that for any $\pi$ and $h\in[H]$, $z_h^{\pi,\phi} \geq \underline{q}$ and
% \begin{align*}
% \underline{p} - z_h^{\pi,\phi} &=\left(\underline{p} - \underline{q}\right)\big(1-\pi_{h}(\phi_{h}\mymid0)\big)=\frac{1}{2}\left(\underline{p} - \underline{q}\right)\big(1-\pi_{h}(\phi_{h}\mymid0)+\pi_{h}(1-\phi_{h}\mymid0)\big) \notag \\
% &=\frac{1}{2}\left(\underline{p} - \underline{q}\right)\big\|\pi_{h}^{\star,\phi}(\cdot\mymid 0)-\pi_{h}(\cdot\mymid 0)\big\|_{1},
% \end{align*}
% and the last inequality arises from \eqref{eq:finite-lb-value-lemma} and \eqref{eq:finite-value-0-lower-bounded}.

% With this in mind, considering the situation when the policy obeying
% \begin{align}
%     \sum_{h=1}^H \big\|\pi_h(\cdot\mymid 0) - \pi_h^{\star, \phi}(\cdot\mymid 0) \big\|_1 \ge \frac{H}{8},
% \end{align}
% applying \eqref{eq:finite-lower-diff} recursively gives
% \begin{align}
%     V_1^{\star, \phi}(0) - V_1^{\pi, \phi}(0) &\geq \frac{1}{12}\sum_{h=1}^H \left(\underline{q}\right)^{h-1} \left(\underline{p} - \underline{q}\right)\big\|\pi_{h}^{\star,\phi}(\cdot\mymid 0)-\pi_{h}(\cdot\mymid 0)\big\|_{1}\left(H-h+1 \right) \notag\\
%     & \overset{\mathrm{(i)}}{\geq} \frac{1}{18} \left(\underline{p} - \underline{q}\right) \sum_{h=1}^H \big\|\pi_{h}^{\star,\phi}(\cdot\mymid 0)-\pi_{h}(\cdot\mymid 0)\big\|_{1}\left(H-h+1 \right) \notag\\
%     & \overset{\mathrm{(ii)}}{>} \frac{1}{18} \left(\underline{p} - \underline{q}\right) \sum_{h =  \left \lceil \frac{15H}{16}\right \rceil}^H (H-h+1) \cdot 2\\
%     & \geq \frac{1}{9} \left(\underline{p} - \underline{q}\right)\left(1+2+\cdots+H+1-\left\lceil \frac{15H}{16}\right\rceil \right)\geq \frac{1}{9} \left(\underline{p} - \underline{q}\right)\frac{\frac{H}{16}(\frac{H}{16}+1)}{2} \notag \\
%     & \geq c_3H \left(\underline{p} - \underline{q}\right)H, \label{eq:finite-lower-diff-result1}
% \end{align}
% for some small enough constant $c_3$.
% where (i) holds by (see \eqref{eq:finite-c2-contraction-bounded})
% \begin{align}
%     \left(\underline{q}\right)^{h-1} \geq \left(\underline{q}\right)^{H} \geq  \left(1-\frac{c_2}{H}\right)^{H} \geq \frac{2}{3},
% \end{align}
% and (ii) holds by borrowing the fact in \cite[Section~C.2.4.]{li2022settling}.

% \paragraph{Step 2: controlling the converted MDP.}
% To further control \eqref{eq:finite-lower-diff-result1}, we first define a auxiliary value functions vector $\overline{V}\in\mathbb{R}^{S\times 1}$ where
% \begin{align}
%     \overline{V}(0) = \alpha H \quad\text{ and } \quad \overline{V}(s) = 0, \quad \forall s\in \cS \setminus  \{0\},
% \end{align}
% where the variable obeys $\alpha\in(0,1]$.
By virtue of \eqref{eq:finite-x-h} and \eqref{eq:finite-lb-value-lemma}, we know that $z_{\phi}^{\star} = \underline{p}$. Applying \eqref{eq:finite-lemma-value-0-pi}, we arrive at
\begin{align}
    \big\langle \rho, V_1^{\star, \phi} - V_1^{\pi, \phi} \big\rangle &= V_h^{\star, \phi}(0) - V_h^{\pi, \phi}(0) = \left(\underline{p} - z_{\phi}^{\pi}\right) (H-1) \notag  = \left(\underline{p} -\underline{q}\right)(H-1)\left(1-\pi_1(\phi\mymid 0)\right), \label{eq:finite-lower-diff}
\end{align}
where the last inequality holds by the definition in \eqref{eq:defination-z-phi-pi}.
Then, we define a auxiliary value functions vector $\overline{V}\in\mathbb{R}^{S\times 1}$ where
\begin{align}
    \overline{V}(0) = (H-1) \quad\text{ and } \quad \overline{V}(s) = 0, \quad \forall s\in \cS \setminus  \{0\}.
\end{align}
With this in hand, applying Lemma~\ref{lem:strong-duality} gives
\begin{align}
    0 \leq  (H-1) \left(\underline{p} - \underline{q}\right) &= \min_{P_{1,0,\phi_h}\in \cB\big(P_{1,0,\phi}^{\phi}, \ror \big)} P_{1,0,1-\phi} \overline{V} -  \min_{P_{1,0,1-\phi}\in \cB\big(P_{1,0,1-\phi}^{\phi}, \ror \big)} P_{1,0,1-\phi} \overline{V} \notag\\
    & = \sup_{\lambda \geq 0}  \left\{ -\lambda \log\left(P_{1,0,\phi}^{\phi} \cdot \exp \left(\frac{-\overline{V}}{\lambda}\right) \right) - \lambda \ror \right\} - \sup_{\lambda \geq 0}  \left\{ -\lambda \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda}\right) \right) - \lambda \ror \right\}\notag\\
    & \overset{\mathrm{(i)}}{\geq}  \left\{ -\lambda^\star  \log\left(P_{1,0,\phi}^{\phi} \cdot \exp \left(\frac{-\overline{V}}{\lambda^\star}\right) \right) - \lambda^\star\ror \right\} -  \left\{ -\lambda^\star \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda^\star}\right) \right) - \lambda^\star \ror\right\} \notag \\
    & = -\lambda^\star \left[\log\left(P_{1,0,\phi}^{\phi} \cdot \exp \left(\frac{-\overline{V}}{\lambda^\star}\right) \right) - \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda^\star}\right) \right)\right]
\end{align}
where (i) holds by letting
\begin{align}
    \lambda^\star \defn \arg \max_{\lambda \geq 0} f(\lambda) \defn \arg \max_{\lambda \geq 0}  \left\{ -\lambda \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda}\right) \right) - \lambda \ror \right\}.
\end{align}
It is easily verified that $\lambda^\star>0$ since $\log(1-q) + \ror \leq  -c_1 (H-1) + 
    \frac{2c_1(H-1)}{3} - 1<0$ (see \eqref{eq:finite-lower-ror-bounded}).

To continue, we have
\begin{align}
    (H-1) \left(\underline{p} - \underline{q}\right) &\geq -\lambda^\star \left[\log\left(P_{1,0,\phi}^{\phi} \cdot \exp \left(\frac{-\overline{V}}{\lambda^\star}\right) \right) - \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda^\star}\right) \right)\right] \notag \\
    & \overset{\mathrm{(i)}}{=} -\lambda^\star \log \frac{p e^{- (H-1)/\lambda^\star} + (1-p)}{q e^{-(H-1)/\lambda^\star} + (1-q)} \notag \\
    & = -\lambda^\star \log \left(1 + \frac{(p-q) \left(e^{-(H-1)/\lambda^\star} -1 \right)}{qe^{-(H-1)/\lambda^\star} + (1-q)} \right) \notag \\
    & \overset{\mathrm{(ii)}}{\geq} \lambda^\star\frac{\Delta  \left(1- e^{-(H-1)/\lambda^\star} \right)}{q e^{-(H-1)/\lambda^\star} + (1-q)} \notag \\
    & = \lambda^\star\frac{\Delta \left( e^{(H-1)/\lambda^\star} -1\right)}{q + (1-q)e^{(H-1)/\lambda^\star}} \notag \\
    & \overset{\mathrm{(iii)}}{\geq} 4 \lambda^\star \Delta \left( e^{(H-1)/\lambda^\star} -1\right) \label{eq:finite-lower-V-diff-bounded}
\end{align}
where (i) follows from the definitions in \eqref{eq:Ph-construction-lower-finite}, 
(ii) holds by $\log(1+x)<x$ for $x\in(-1,\infty)$ and $\lambda^\star>0$, (iii) is verified by the following fact whose proof is postponed to the end
\begin{align}\label{eq:finite-lower-check-lambda-star}
   \frac{1}{2} e^{-12(H-1)/7\lambda^\star} \leq 1-p\leq 1-q \leq 3e^{-(H-1)/\lambda^\star} \quad \text{ and } \quad \lambda^\star \geq \frac{1}{c_1} \geq \frac{3H}{2\ror}.
\end{align}


Finally, inserting \eqref{eq:finite-lower-V-diff-bounded} back into \eqref{eq:finite-lower-diff} yields 
\begin{align}
\big\langle \rho, V_1^{\star, \phi} - V_1^{\pi, \phi} \big\rangle &= V_1^{\star, \phi}(0) - V_1^{\pi, \phi}(0) \geq 4 \lambda^\star \Delta \left( e^{(H-1)/\lambda^\star} -1\right) \left(1-\pi_1(\phi\mymid 0)\right)\geq 2\varepsilon \left(1-\pi_1(\phi\mymid 0)\right),
\end{align}
which holds by choosing 
\begin{align}
    \Delta = \frac{\ror \varepsilon}{ 6H \left( e^{(H-1)/\lambda^\star} -1\right)} \geq \frac{\varepsilon}{ 4\lambda^\star \left( e^{(H-1)/\lambda^\star} -1\right)}. 
\end{align}
\paragraph{Proof of inequality \eqref{eq:finite-lower-check-lambda-star}.}
% First, we introduce some useful notations
% \begin{align}
%     p_0 \defn \mu(0) + p\mu(1),\qquad q_0 = \mu(0) + q\mu(1).
% \end{align}
\paragraph{Step 1: showing the first assertion.}
To begin with, Recalling the facts of $\lambda^\star$ and $\ror$ in \eqref{eq:finite-lower-ror-bounded} and \eqref{eq:lambda-n-range}, we have
\begin{align}
    \lambda^\star \leq \frac{H-1}{\ror} \leq \frac{H-1}{\frac{2c_1 (H-1)}{3} - 1} \leq \frac{H-1}{\frac{7c_1 (H-1)}{12}} = \frac{12}{7c_1},
\end{align}
where the penultimate inequality holds by choosing $\frac{c_1 (H-1)}{12}\geq 1$.

Therefore, we finally arrive at
\begin{align}
    1- p \geq \frac{1}{2} e^{-c_1(H-1)} \geq \frac{1}{2} e^{-12(H-1)/7\lambda^\star}.
\end{align}
% In addition, when it comes to
% \begin{align}
%     \frac{3}{4}(e^{-c_1H} -\Delta) \leq 1- p_0 = \mu(1)(1-p) \defn c_p e^{-H/\lambda_p}. 
% \end{align}

% So 
% \begin{align}
%     \nabla_\lambda f(\lambda) \mymid_{\lambda =\lambda_p} &= -\ror(\Phi) - \log(1-p_0) - \log\left( 1 + \frac{p_0}{c_p}\right) + \frac{p_0/c_p }{p_0/c_p + 1} \notag\\
%     & \overset{\mathrm{(i)}}{\leq} -\ror(\Phi) + c_5 H - \log\left( 1 + \frac{p_0}{c_p}\right) + \frac{p_0/c_p }{p_0/c_p + 1} \\
%     & \leq -\ror(\Phi) + c_5 H - \log 2 + \frac{1}{3} \leq 0
% \end{align}
% $c_5\geq c_1$



\paragraph{Step 2: showing the third assertion.}
Next, we shall focus on showing
\begin{align}
    1- q \leq 3e^{-(H-1)/\lambda^\star}. 
\end{align}

Recalling \eqref{eq:finite-p-q-def} and \eqref{eq:lambda-n-range}, with positive variables $c_q$ and $\lambda_q$, we can reparameterize $1-q$ as follows:
\begin{align}
1- q = e^{-c_1 (H-1)} = c_q e^{-(H-1)/\lambda_q}. \label{eq:assumption-of-q-0}
\end{align}

Invoking the first derivative of the function of interest is 
\begin{align}
    \nabla_\lambda f(\lambda) &= \left( -\lambda \log\left(P_{1,0,1-\phi}^{\phi} \cdot \exp \left(\frac{- \overline{V}}{\lambda}\right) \right) - \lambda \ror \right) \notag\\
    & = \nabla_\lambda \left( -\lambda \log\left(q e^{-(H-1)/\lambda} + 1-q\right) - \lambda \ror \right) \notag\\
    & = -\ror -\log \left(q e^{-(H-1)/\lambda} + 1-q\right) + \frac{q\frac{-(H-1)}{\lambda}e^{-(H-1)/\lambda} }{q e^{-(H-1)/\lambda} + 1-q}.
    \end{align}

To continue, plugging in \eqref{eq:assumption-of-q-0}, when $\lambda = \lambda_q$, the derivative of the function is
\begin{align}
     \nabla_\lambda f(\lambda) \mymid_{\lambda =\lambda_q} &= -\ror - \log\left[ (1-q)\frac{q}{c_q}  + 1 - q\right] + \frac{(1-q)\frac{q}{c_q} \log\frac{1-q}{c_q} }{(1-q)\frac{q}{c_q}   + 1-q} \notag \\
    & = -\ror - \log(1-q) - \log\left( 1 + \frac{q}{c_q} \right) + \frac{\frac{q}{c_q} \log\frac{1-q}{c_q} }{\frac{q}{c_q}   + 1} \notag \\
    & = -\ror - \log(1-q)\left[1 -\frac{q/c_q}{q/c_q + 1}\right] - \log\left( 1 + \frac{q}{c_q} \right) - \frac{ q/c_q\log(c_q)}{1 + q/c_q }  \notag \\
    & \overset{\mathrm{(i)}}{=} -\ror + c_1 (H-1)\left[1 -\frac{q/c_q}{q/c_q + 1}\right] - \log\left( 1 + \frac{q}{c_q} \right) - \frac{ q/c_q\log(c_q)}{1 + q/c_q }  \\
    & \overset{\mathrm{(ii)}}{\geq} -\frac{2c_1 (H-1)}{3} + \frac{3c_1 (H-1)}{4} - \log2 - \frac{\log 3}{4}\notag \\
    &  \geq \frac{c_1 (H-1)}{12} - 2\geq 0
\end{align}
where (i) holds by \eqref{eq:assumption-of-q-0}, (ii) follows from choosing $c_q = 3$, the fact $1/3\leq q \leq 1$, and the fact of $\ror$ in \eqref{eq:finite-lower-ror-bounded}. Here, the last inequality holds by letting $H \geq \frac{24}{c_1} + 1$.

Note that the function $f(\lambda)$ is concave with respect to $\lambda$. Therefore, since $\nabla_\lambda f(\lambda) \mymid_{\lambda =\lambda_q} \geq 0$, we have $\lambda_q \leq \lambda^\star$, which implies
\begin{align}
    1- q= c_q e^{-(H-1) /\lambda_q} \leq 3e^{-(H-1) /\lambda^\star}.
\end{align}

In addition, $e^{-c_1(H-1)} \leq 3e^{-(H-1) /\lambda^\star}$ and the fact of $\ror$ in \eqref{eq:finite-lower-ror-bounded} directly verify
\begin{align}
    \lambda^\star \geq \frac{1}{c_1 \log3}\geq \frac{1}{2 c_1} \geq \frac{3H}{2 \ror},
\end{align}
with $H$ properly chosen.


% we note that  
% for any $0\leq a_{1}\leq a_{2}\leq\cdots\leq a_{H}$ 
% and any $0\leq x_{1},\cdots, x_{H}\leq x_{\max}$
% obeying $\sum_{i=1}^{H}x_{i}\geq x_{\text{sum}}$,
% the following elementary inequality holds: 
% %
% \[
%     \sum_{i=1}^{H}x_{i}a_{i}\geq\sum_{i=1}^{\lfloor x_{\text{sum}}/ x_{\max} \rfloor}x_{\max}a_{i};
% \]
% %
% this together with $\big\|\pi_h^{\star, \theta}(\cdot\mymid 0) - \pi_h(\cdot\mymid 0)\big\|_1\leq 2$ and \eqref{eq:finite-lower-delta} validates the inequality (ii). 


==> preliminary.tex <==
\section{Technical lemmas}
\subsection{Preliminary facts}
Our results rely heavily on proper choices of the learning rates. In what follows, 
we make note of several useful properties concerning the learning rates, which have been established in \cite{jin2018q,li2021breaking}.
%
\begin{lemma}[Lemma 1 in \citep{li2021breaking}]
	\label{lemma:property of learning rate} 
	For any integer $N>0$, the following properties hold:
%
\begin{subequations}
\label{eq:properties-learning-rates}
%
\begin{align}
	& \frac{1}{N^a}  \le\sum_{n=1}^{N}\frac{\eta_{n}^{N}}{n^a}\le\frac{2}{N^a} \qquad \mbox{for all}\quad  \frac{1}{2} \leq a \leq 1,
	\label{eq:properties-learning-rates-12}\\
\max_{1\le n\le N} & \eta_{n}^{N}\le\frac{2H}{N},\qquad\sum_{n=1}^{N}(\eta_{n}^{N})^{2}\le\frac{2H}{N}, \qquad
	 \sum_{N=n}^{\infty}\eta_{n}^{N}\le1+\frac{1}{H}.
	 \label{eq:properties-learning-rates-345}
\end{align}
%
\end{subequations}
 
\end{lemma}
%

In addition, we gather a few elementary properties about the Binomial distribution, which will be useful throughout the proof.
The lemma below is adapted from \citet[Lemma A.1]{xie2021policy}. 
\begin{lemma}\label{lem:binomial} 
  Suppose $N\sim \mathsf{Binomial}(n,p)$, where $n\geq 1$ and $p\in [0,1]$. For any $\delta\in (0,1)$, we have
  \begin{align}
    \frac{p}{N\vee 1} &\leq \frac{8\log\left(\frac{1}{\delta}\right)}{n},  \label{equ:binomial}
  \end{align}
and 
\begin{subequations}
  \label{equ:binomial-all}
  \begin{align}
    N&\geq \frac{np}{8\log\left(\frac{1}{\delta}\right)} \qquad \text{ if } np \geq 8\log\left(\frac{1}{\delta}\right), \label{equ:binomial2}\\
    N &\leq \begin{cases}
 e^2np & \text{ if } np \geq \log\left(\frac{1}{\delta}\right), \\ 
2e^2 \log\left(\frac{1}{\delta}\right) & \text{ if } np \leq 2\log\left(\frac{1}{\delta}\right).
\end{cases} \label{equ:binomial3}
  \end{align}
\end{subequations}
%
  with probability at least $1 - 4\delta$. 
 
\end{lemma}
%
\begin{proof}
To begin with, we directly invoke \citet[Lemma A.1]{xie2021policy} which yields the results in \eqref{equ:binomial} and \eqref{equ:binomial2}. Regarding \eqref{equ:binomial3}, invoking the Chernoff bound \citep[Theorem 2.3.1]{vershynin2018high} with $\mathbb{E}[N] = np$, when $np \geq \log\left(\frac{1}{\delta}\right)$, it satisfies
\begin{align*}
\mathbb{P}(N \geq e^2np) &\leq e^{-np}\left(\frac{enp}{e^2np}\right)^{ e^2np} \leq e^{-np} \leq \delta.
\end{align*}
Similarly, when $ np \leq 2\log\left(\frac{1}{\delta}\right)$, we have
\begin{align*}
\mathbb{P}\left(N \geq 2e^2\log\left(\frac{1}{\delta}\right)\right)& \overset{\mathrm{(i)}}{\leq} 
e^{-np}\left(\frac{enp}{2e^2\log\left(\frac{1}{\delta}\right)}\right)^{ 2e^2\log(\frac{1}{\delta})} \\
&\overset{\mathrm{(ii)}}{\leq} e^{-np}\left(\frac{enp}{e^2np}\right)^{ 2e^2\log(\frac{1}{\delta})} \leq e^{-2e^2 \log\left(\frac{1}{\delta}\right)} \leq \delta,
  \end{align*}
where (i) results from \citet[Theorem 2.3.1]{vershynin2018high}, and (ii) follows from the basic fact $e^2\log\left(\frac{1}{\delta}\right) \geq 2\log\left(\frac{1}{\delta}\right) \geq np$. 
Taking the union bound thus completes the proof. 
\end{proof}






\subsection{Freedman's inequality and its consequences}


Both the samples collected within each episode and the algorithms analyzed herein exhibit certain Markovian structure. 
As a result, concentration inequalities tailored to martingales become particularly effective for our analysis. 
In this subsection, we collect a few useful concentration results that will be applied multiple times in the current paper. These results might be of independent interest.



To begin with, the following theorem provides a user-friendly version of Freedman's
inequality \citep{freedman1975tail}; 
see \citet[Section C]{li2021tightening} for more details.
%
\begin{theorem}[Freedman's inequality]\label{thm:Freedman}
Consider a filtration $\mathcal{F}_0\subset \mathcal{F}_1 \subset \mathcal{F}_2 \subset \cdots$,
and let $\mathbb{E}_{k}$ stand for the expectation conditioned
on $\mathcal{F}_k$. 
Suppose that $Y_{n}=\sum_{k=1}^{n}X_{k}\in\mathbb{R}$,
where $\{X_{k}\}$ is a real-valued scalar sequence obeying
\[
  \left|X_{k}\right|\leq R\qquad\text{and}\qquad\mathbb{E}_{k-1} \big[X_{k}\big]=0\quad\quad\quad\text{for all }k\geq1
\]
%
for some quantity $R<\infty$. 
We also define
\[
W_{n}\coloneqq\sum_{k=1}^{n}\mathbb{E}_{k-1}\left[X_{k}^{2}\right].
\]
%
In addition, suppose that $W_{n}\leq\sigma^{2}$ holds deterministically for some given quantity $\sigma^2<\infty$.
Then for any positive integer $m \geq1$, with probability at least $1-\delta$
one has
\begin{equation}
\left|Y_{n}\right|\leq\sqrt{8\max\Big\{ W_{n},\frac{\sigma^{2}}{2^{m}}\Big\}\log\frac{2m}{\delta}}+\frac{4}{3}R\log\frac{2m}{\delta}.\label{eq:Freedman-random}
\end{equation}
\end{theorem}







We shall also record some immediate consequence of Freedman's inequality tailored to our problem.  
Recall that $N_h^i(s,a)$ denotes the number of times that $(s,a)$ has been visited at step $h$ before the beginning of the $i$-th episode, 
and $k^n(s,a)$ stands for the index of the episode in which $(s,a)$ is visited for the $n$-th time. The following concentration bound has been established in \citet[Lemma 7]{li2021breaking}.




\begin{lemma}
  \label{lemma:martingale-union-all}
  Let $\big\{ W_{h}^{i} \in \mathbb{R}^S \mid 1\leq i\leq K, 1\leq h \leq H+1 \big\}$ and $\big\{u_h^i(s,a,N)\in \mathbb{R} \mid 1\leq i\leq K, 1\leq h \leq H+1 \big\}$  be a collections of vectors and scalars, respectively, and suppose that they obey the following properties:
  %
  \begin{itemize}
    \item $W_{h}^{i}$ is fully determined by the samples collected up to the end of the $(h-1)$-th step of the $i$-th episode;  
    \item $\|W_h^i\|_{\infty}\leq C_\mathrm{w}$; 
    \item $u_h^i(s,a, N)$  is fully determined by the samples collected up to the end of the $(h-1)$-th step of the $i$-th episode, and a given positive integer $N\in[K]$;
    \item $0\leq u_h^i(s,a, N) \leq C_{\mathrm{u}}$;
    \item $0\leq \sum_{n=1}^{N_h^k(s,a)} u_h^{k_h^n(s,a)}(s,a, N) \leq 2$.  
    
  \end{itemize}
  %
  In addition, consider the following sequence  
  \begin{align}
    X_i (s,a,h,N) &\defn u_h^i(s,a, N) \big(P_h^{i} - P_{h,s,a}\big) W_{h+1}^{i} 
    \ind\big\{ (s_h^i, a_h^i) = (s,a)\big\},
    \qquad 1\leq i\leq K,  
  \end{align}
  with $P_h^{i}$ defined in \eqref{eq:Phk_def}. 
  Consider any $\delta \in (0,1)$. Then with probability at least $1-\delta$, 
  %
  \begin{align}
    & \left|\sum_{i=1}^k X_i(s,a,h,N) \right| \notag\\
    & \quad \lesssim \sqrt{C_{\mathrm{u}} \log^2\frac{SAT}{\delta}}\sqrt{\sum_{n = 1}^{N_h^k(s,a)} u_h^{k_h^n(s,a)}(s,a,N) \Var_{h, s,a} \big(W_{h+1}^{k_h^n(s,a)}  \big)} + \left(C_{\mathrm{u}} C_{\mathrm{w}} + \sqrt{\frac{C_{\mathrm{u}}}{N}} C_{\mathrm{w}}\right) \log^2\frac{SAT}{\delta}
  \end{align}
  %
  holds simultaneously for all $(k, h, s, a, N) \in [K] \times [H] \times \cS \times \cA \times [K]$.  
\end{lemma}


Next, we make note of an immediate consequence of Lemma~\ref{lemma:martingale-union-all} as follows.
%
\begin{lemma}\label{lemma:azuma-hoeffding}
Let $\big\{ W_{h}^{i} \in \mathbb{R}^S \mid 1\leq i\leq K, 1\leq h \leq H+1 \big\}$ be a collection of vectors satisfying the following properties: 
  \begin{itemize}
    \item $W_{h}^{i}$ is fully determined by the samples collected up to the end of the $(h-1)$-th step of the $i$-th episode;  
    \item $\|W_h^i\|_{\infty}\leq C_\mathrm{w}$.
  \end{itemize}

For any positive $N \geq H$, we consider the following sequence 
\begin{align}
  X_i(s,a,h,N) &\defn \eta_{N_h^i(s,a)}^N \big(P_h^{i} - P_{h,s,a}\big) W_{h+1}^{i}
    \ind\big\{ (s_h^i, a_h^i) = (s,a)\big\},
    \qquad 1\leq i\leq K,
\end{align}
%
with $P_h^{i}$ defined in \eqref{eq:Phk_def}. 
Consider any $\delta\in (0,1)$. With probability at least $1-\delta$, 
%
  \begin{align}
    & \left|\sum_{i=1}^k X_i(s,a,h,N) \right| \lesssim \sqrt{\frac{H}{N} C_{\mathrm{w}}^2 }\log^2\frac{SAT}{\delta} 
  \end{align}
%
holds simultaneously for all $(k, h, s, a, N) \in [K] \times [H] \times \cS \times \cA \times [K]$.  
\end{lemma}
%
\begin{proof}
%
Taking $u_{h}^{i}(s,a,N)=\eta_{N_{h}^{i}(s,a)}^{N}$, one can see from \eqref{eq:properties-learning-rates-345} in Lemma~\ref{lemma:property of learning rate} that
%
\[
	\big|u_{h}^{i}(s,a,N)\big|\leq\frac{2H}{N}\eqqcolon C_{\mathrm{u}}.
\]
%
Recognizing the trivial bound $\Var_{h,s,a}\big(W_{h+1}^{k_{h}^{n}(s,a)}\big)\leq C_{\mathrm{w}}^{2}$,
we can invoke Lemma~\ref{lemma:martingale-union-all} to obtain that, with probability at least $1-\delta$, 
\begin{align*}
  \Bigg|\sum_{i=1}^{k}X_{i}(s,a,h,N)\Bigg|
 & \lesssim\sqrt{C_{\mathrm{u}}\log^{2}\frac{SAT}{\delta}}\sqrt{\sum_{n=1}^{N_{h}^{k}(s,a)}\eta_{n}^{N}C_{\mathrm{w}}^{2}}+\left(C_{\mathrm{u}}C_{\mathrm{w}}+\sqrt{\frac{C_{\mathrm{u}}}{N}}C_{\mathrm{w}}\right)\log^{2}\frac{SAT}{\delta}\\
 & \lesssim\sqrt{\frac{H}{N}\log^{2}\frac{SAT}{\delta}}\cdot C_{\mathrm{w}}+\frac{HC_{\mathrm{w}}}{N}\log^{2}\frac{SAT}{\delta}\lesssim\sqrt{\frac{HC_{\mathrm{w}}^{2}}{N}}\log^{2}\frac{SAT}{\delta}
\end{align*}
holds simultaneously for all $(k, h, s, a, N) \in [K] \times [H] \times \cS \times \cA \times [K]$, where the last line applies \eqref{eq:properties-learning-rates-345} in Lemma~\ref{lemma:property of learning rate} once again.
%
\end{proof}



Finally, we introduce another lemma by invoking Freedman's inequality in Theorem~\ref{thm:Freedman}.
\begin{lemma}
  \label{lemma:martingale-union-recursion}
  Let $\big\{ W_{h}^{k}(s,a) \in \mathbb{R}^S \mid (s,a)\in\cS\times \cA, 1\leq k\leq K, 1\leq h \leq H+1 \big\}$ be a collection of vectors satisfying the following properties: 
  \begin{itemize}
    \item $W_{h}^{k}(s,a)$ is fully determined by the given state-action pair $(s,a)$ and the samples collected up to the end of the $(k-1)$-th episode;  
    \item $\|W_h^k(s,a)\|_{\infty}\leq C_\mathrm{w}$.
  \end{itemize}

For any positive $ C_{\mathrm{d}} \geq 0$, we consider the following sequences 
\begin{align}
  X_{h,k} &\defn C_{\mathrm{d}} \left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_{h,s_h^k,a_h^k}W_{h+1}^{k}(s_h^k,a_h^k) - \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}W_{h+1}^{k}(s,a)\right],
    \qquad 1\leq k\leq K,\\
  \overline{X}_{h,k} &\defn C_{\mathrm{d}} \left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_{h}^k W_{h+1}^{k}(s_h^k,a_h^k) - \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}W_{h+1}^{k}(s,a)\right],
    \qquad 1\leq k\leq K.
\end{align}
  Consider any $\delta \in (0,1)$. Then with probability at least $1-\delta$, 
  %
  \begin{align}
    & \left|\sum_{k=1}^K X_{h,k}\right| \leq \sqrt{\sum_{k=1}^K 8 C_{\mathrm{d}}^2 C^\star \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) \left[P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \log\frac{2H}{\delta}} + 2C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta} \\
  &\left|\sum_{k=1}^K \overline{X}_{h,k}\right| \leq \sqrt{\sum_{k=1}^K 8 C_{\mathrm{d}}^2 C^\star \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}\left[W_{h+1}^{k}(s,a)\right]^2 \log\frac{2H}{\delta}} + 2C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta}
  \end{align}
  %
  hold simultaneously for all $h\in[H]$.  
\end{lemma}
\begin{proof}
We intend to apply Freedman's inequality (cf.~Theorem~\ref{thm:Freedman}) to control $\sum_{k=1}^K X_{h,k}$. Considering any given time step $h$, it is easily verified that
  \begin{align*}
    \mathbb{E}_{k-1}[X_{h,k}] =0, \qquad \mathbb{E}_{k-1}[\overline{X}_{h,k}] =0,
  \end{align*}
where $\mathbb{E}_{k-1}$ denotes the expectation conditioned on everything happening up to the end of the $(k-1)$-th episode. To continue, we observe that
\begin{align}
  |X_{h,k}| \leq C_{\mathrm{d}}\left(\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} + 1\right) \left\|W_{h+1}^k(s,a)\right\|_\infty  \leq 2C_{\mathrm{d}} C^\star C_\mathrm{w}, \label{eq:X-R}\\
  |\overline{X}_{h,k}| \leq C_{\mathrm{d}}\left(\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} + 1\right) \left\|W_{h+1}^k(s,a)\right\|_\infty  \leq 2C_{\mathrm{d}} C^\star C_\mathrm{w}, \label{eq:X-R-2}
\end{align}
	where we use the assumptions $\frac{d_{h}^{\pi_{\star}}(s,a)}{d_{h}^{\mu}(s,a)} \leq C^\star$ for all $(h,s,a)\in[H]\times \cS\times \cA$ (cf.~Assumption~\ref{assumption}) and $\left\|W_{h+1}^k(s_h^k,a_h^k)\right\|_\infty  \leq C_{\mathrm{w}}$. 

Recall that $\Delta(\cS \times \cA)$ is the probability simplex over the set $\cS\times \cA$ of all state-action pairs, and we denote by $d_h^{\mu} \in \Delta(\cS \times \cA)$  the state-action visitation distribution induced by the behavior policy $\mu$ at time step $h\in[H]$. 
With this in hand, we obtain
\begin{align}
  \sum_{k=1}^K \mathbb{E}_{k-1}[|X_{h,k}|^2] &\leq \sum_{k=1}^K C_{\mathrm{d}}^2 \mathbb{E}_{k-1}\left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_{h,s_h^k,a_h^k}W_{h+1}^{k}(s_h^k,a_h^k) - \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \nonumber\\
  & \leq \sum_{k=1}^K C_{\mathrm{d}}^2 \mathbb{E}_{(s_h^k,a_h^k) \sim d_h^\mu}\left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_{h,s_h^k,a_h^k}W_{h+1}^{k}(s_h^k,a_h^k)\right]^2 \nonumber\\
  & = \sum_{k=1}^K C_{\mathrm{d}}^2 \sum_{(s,a)\in\cS\times\cA} \frac{d_{h}^{\pi_{\star}}(s,a)}{d_{h}^{\mu}(s,a)}d_{h}^{\pi_{\star}}(s,a) \left[P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \nonumber\\
  & \overset{\mathrm{(i)}}{\leq} \sum_{k=1}^K C_{\mathrm{d}}^2 C^\star\sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) \left[P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \label{eq:var-of-w}  \\
  &\leq \sum_{k=1}^K C_{\mathrm{d}}^2 \sum_{(s,a)\in \cS\times\cA}C^\star d_{h}^{\pi_{\star}}(s,a) \left\|W_{h+1}^k(s_h^k,a_h^k)\right\|_\infty^2 \leq C_{\mathrm{d}}^2 C^\star C_{\mathrm{w}}^2 K, \label{eq:var-of-w-crude}
\end{align}
where (i) follows from $\frac{d_{h}^{\pi_{\star}}(s,a)}{d_{h}^{\mu}(s,a)} \leq C^\star$ (see Assumption~\ref{assumption}) and the assumption $\left\|W_{h+1}^k(s_h^k,a_h^k)\right\|_\infty  \leq C_{\mathrm{w}}$.

Similarly, we can derive
\begin{align}
  \sum_{k=1}^K \mathbb{E}_{k-1}[|\overline{X}_{h,k}|^2] &\leq \sum_{k=1}^K C_{\mathrm{d}}^2 \mathbb{E}_{k-1}\left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_h^k W_{h+1}^{k}(s_h^k,a_h^k) - \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \nonumber\\
  & \leq \sum_{k=1}^K C_{\mathrm{d}}^2 \mathbb{E}_{(s_h^k,a_h^k) \sim d_h^\mu} \left[ \mathbb{E}_{P_h^k \sim P_{h,s_h^k,a_h^k}}  \left[\frac{d_{h}^{\pi_{\star}}(s_h^k,a_h^k)}{d_{h}^{\mu}(s_h^k,a_h^k)} P_h^k W_{h+1}^{k}(s_h^k,a_h^k)\right]^2 \right] \nonumber\\
  & = \sum_{k=1}^K C_{\mathrm{d}}^2 \sum_{(s,a)\in\cS\times\cA} \frac{d_{h}^{\pi_{\star}}(s,a)}{d_{h}^{\mu}(s,a)}d_{h}^{\pi_{\star}}(s,a) \mathbb{E}_{P_h^k \sim P_{h,s,a}}\left[P_h^k W_{h+1}^{k}(s,a)\right]^2 \nonumber\\
  & \overset{\mathrm{(i)}}{\leq} \sum_{k=1}^K C_{\mathrm{d}}^2 C^\star\sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) \mathbb{E}_{P_h^k \sim P_{h,s,a}}\left[P_h^k W_{h+1}^{k}(s,a)\right]^2  \label{eq:var-of-w-2}\\
  & = \sum_{k=1}^K C_{\mathrm{d}}^2 C^\star\sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}\left[W_{h+1}^{k}(s,a)\right]^2  \label{eq:var-of-w-2}\\
  &\leq \sum_{k=1}^K C_{\mathrm{d}}^2 \sum_{(s,a)\in \cS\times\cA}C^\star d_{h}^{\pi_{\star}}(s,a) \left\|W_{h+1}^k(s,a)\right\|_\infty^2 \leq C_{\mathrm{d}}^2 C^\star C_{\mathrm{w}}^2 K, \label{eq:var-of-w-crude-2}
\end{align}
where (i) follows from $\frac{d_{h}^{\pi_{\star}}(s,a)}{d_{h}^{\mu}(s,a)} \leq C^\star$ (see Assumption~\ref{assumption}) and the assumption $\left\|W_{h+1}^k(s_h^k,a_h^k)\right\|_\infty  \leq C_{\mathrm{w}}$.

Plugging in the results in \eqref{eq:X-R} and \eqref{eq:var-of-w} (resps.~\eqref{eq:X-R-2} and \eqref{eq:var-of-w-2}) to control $\sum_{k=1}^K \left|X_{h,k}\right|$ (resps.~$\sum_{k=1}^K \left|\overline{X}_{h,k}\right|$), we invoke Theorem~\ref{thm:Freedman} with $m=\lceil \log_2 K \rceil$ and take the union bound over $h\in[H]$ to show that with probability at least $1-\delta$,
\begin{align}
  \left|\sum_{k=1}^K X_{h,k}\right|& \leq\sqrt{8\max\left\{\sum_{k=1}^K C_{\mathrm{d}}^2C^\star \sum_{(s,a)\in\cS\times\cA}d_{h}^{\pi_{\star}}(s,a) \left[P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2, \frac{C_{\mathrm{d}}^2 C^\star C_{\mathrm{w}}^2 K}{2^m}\right\} \log\frac{2H}{\delta}} \nonumber \\
  &\qquad + \frac{8}{3}C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta} \nonumber \\
  &\leq \sqrt{\sum_{k=1}^K 8 C_{\mathrm{d}}^2 C^\star \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) \left[P_{h,s,a}W_{h+1}^{k}(s,a)\right]^2 \log\frac{2H}{\delta}} + 6C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta} \nonumber
\end{align}
and
\begin{align}
  \left|\sum_{k=1}^K \overline{X}_{h,k}\right|& \leq\sqrt{8\max\left\{\sum_{k=1}^K C_{\mathrm{d}}^2C^\star \sum_{(s,a)\in\cS\times\cA}d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}\left[W_{h+1}^{k}(s,a)\right]^2, \frac{C_{\mathrm{d}}^2 C^\star C_{\mathrm{w}}^2 K}{2^m}\right\} \log\frac{2H}{\delta}} \nonumber \\
  &\qquad + \frac{8}{3}C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta} \nonumber \\
  &\leq \sqrt{\sum_{k=1}^K 8 C_{\mathrm{d}}^2 C^\star \sum_{(s,a)\in\cS\times\cA} d_{h}^{\pi_{\star}}(s,a) P_{h,s,a}\left[W_{h+1}^{k}(s,a)\right]^2 \log\frac{2H}{\delta}} + 6C_{\mathrm{d}} C^\star C_\mathrm{w}\log\frac{2H}{\delta} \nonumber
\end{align}
holds simultaneously for all $h\in[H]$.
\end{proof}


==> upper-bound-analysis-exp.tex <==
%!TEX root = ./DRO-offline.tex
\section{Analysis}\label{sec:analysis}
% \subsection{Proof of Theorem~\ref{thm:dro-upper-finite}}

To start with, we shall introduce several notations that is useful in showing the main results. We introduce the notations about the minimum of the nonnegative entries in transition kernels as
\begin{align}
	P_{\min,h}\left(s, a\right) \defn \min_{s': P^{\no}_h(s' \mymid s,a)>0 } P^{\no}_h(s' \mymid s,a),\qquad
	\minpall \defn \min_{(h,s)\in[H]\times\cS} P_{\min,h}\left(s, \pi_h^\star(s)\right).
\end{align}
Note that $P_{\min,h}$ and $\minpall$ are fully determined by the nominal MDP $P^{\no}$ (independent of $\cD)$. 

In addition, for all $(h,s,a)$, we denote the dual problem solutions and their minimum as
\begin{align}\label{eq:defn-lambda-star}
	&\lambda_{h,s,a}^\star \defn \arg \max_{\lambda\geq 0}  \left\{ -\lambda \log\left(P^{\no}_{h, s, a} \cdot \exp \left(\frac{-\widehat{V}_{h+1}}{\lambda}\right) \right) - \lambda \ror \right\}, \qquad \lambda^\star \defn \min_{(h,s)\in [H]\times \cS} \lambda^\star_{h,s,\piopt_h(s)}
\end{align}
which are determined by $P^{\no}$ and the estimation $\{\widehat{V}_{h+1}\}_{h=1}^H$.

We sketch the proof outline of Theorem~\ref{thm:dro-upper-finite}, which is separated into several steps.

Before starting, we introduce several additional useful notations. Let $\mathrm{ess}\inf X \defn \sup\{x: X(s)\geq x\}$ denote the essential infimum of any vector $X\in \mathbb{R}^S$. In addition, we denote the coverage state-action space by the dataset $\cD_0$ as follows
\begin{equation}
	\cC_{\pib} = \{(h,s,a): N_h(s,a) >0\}.
\end{equation}
% Before starting, more generally, for any nominal distribution $P^0\in \Delta(\cS)$, the uncertainty set with radius $\delta$ is defined similar to \eqref{eq:kl-ball-finite-P} as \yc{change the notation $P^0$ since it is the transition kernel}
% \begin{align}
% 	\cB(P^0,\delta) \defn \left\{ P \in \Delta (\cS): \mathsf{KL}(P \parallel P^0) \leq \delta \right\}.
% \end{align}

\paragraph{Step 1: establishing the pessimism property $\widehat{Q}_h(s,a) \leq Q^{\widehat{\pi},\sigma}_h(s,a)$.} 
 
To achieve this claim, we heavily count on the following lemma.
\begin{lemma}\label{lemma:dro-b-bound}
Consider any $(h,s,a)\in [H] \times\cS\times\cA$ and any vector $V\in \mathbb{R}^S$ independent of $\widehat{P}^0_{h,s,a}$ and $P^{\no}_{h,s,a}$ obeying $\|V\|_{\infty} \le H-h+1$. 
	With probability at least $1- \frac{\delta}{KH}$, one has
\begin{align}
	&\left|\inf_{ \cP \in \unb^{\sigma}(\widehat{P}_{h,s,a}^0)} \cP V - \inf_{ \cP \in \unb^{\sigma}(P^{\no}_{h,s,a})}  \cP V \right| \leq b_h (s,a  \mymid V ),
\end{align}
as long as 
\begin{align}
N_h(s,a) \geq N_h(s,a, V, \ror) \defn c_1 \max\left \{\frac{\log\frac{KH}{\delta}  \cdot \mathbb{P}_{s\sim P^{\no}_{h,s,a}}(V(s)= \mathrm{ess}\inf V) }{ \big(\mathbb{P}_{s\sim P^{\no}_{h,s,a}}(V(s)= \mathrm{ess}\inf V) - e^{-\ror} \big)^2}, \frac{H^2 \exp(8H/\lambda^\star_{h,s,a})}{\tau^2 \ror^2} \log\frac{6KH}{\delta}\right\}.
\end{align}
Here $\tau$ is some parameter depend on $\lambda^\star, P^{\no}_{h,s,a}, \ror, V$. \lxs{The term $ N_h(s,a, V, \ror)$ is determined by $\lambda^\star, P^{\no}_{h,s,a}, \ror, V$ but not $\varepsilon$.}
\end{lemma}
\begin{proof}
See Appendix~\ref{proof:lemma:dro-b-bound}.
\end{proof}

Applying above lemma directly with $V =\widehat{V}_{h+1}$ (which is independent of $\widehat{P}^{\no}_{h,s,a}$) indicates that with probability at least $1-\delta$,
\begin{align}\label{eq:dro-b-bound}
	\left|\inf_{ \cP \in \unb^{\sigma}(\widehat{P}_{h,s,a}^0)} \cP \widehat{V}_{h+1} - \inf_{ \cP \in \unb^{\sigma}(P^{\no}_{h,s,a})}  \cP \widehat{V}_{h+1} \right| \leq b_h (s,a).
\end{align}
holds for all $(h,s,a)\in \cC_{\pib}$ as long as
\begin{align}\label{eq:dro-b-bound-N-condition}
	N &\geq \sum_{(h,s,a)\in \cC_{\pib}} N_h(s,a, \widehat{V}_{h+1}, \ror)\notag \\
	& \geq \max_{(h,s,a)\in \cC_{\pib}}\max\left \{\frac{c_1|\cC_{\pib}| \log\frac{KH}{\delta}  \cdot \mathbb{P}_{s\sim P^{\no}_{h,s,a}}\left[\widehat{V}_{h+1}(s)= \mathrm{ess}\inf \widehat{V}_{h+1}\right] }{ \left[\mathbb{P}_{s\sim P^{\no}_{h,s,a}}(\widehat{V}_{h+1}(s)= \mathrm{ess}\inf \widehat{V}_{h+1}) - e^{-\ror} \right]^2}, \frac{c_1|\cC_{\pib}|  H^2 \exp(8H/\lambda^\star_{h,s,a})}{\tau^2 \ror^2} \log\frac{6KH}{\delta}\right\}.
\end{align}


Armed with above facts,  we shall show that, with probability at least $1-\delta$, the following relation holds 
\begin{align}\label{eq:finite-pessimism-assertion}
	&\forall (s,a,h) \in \cS\times \cA\times [H+1]:
	\qquad \widehat{Q}_h(s,a) \leq Q^{\widehat{\pi},\ror}_h(s,a),\qquad \widehat{V}_h(s) \leq V^{\widehat{\pi},\ror}_h(s).
\end{align}
Towards this, it is easily verified that the latter assertion concerning $V^{\widehat{\pi},\ror}_h$ is implied by the former, since
\begin{align}
	\widehat{V}_h(s) = \max_a \widehat{Q}_h(s, a) \leq \max_a Q^{\widehat{\pi},\ror}_h(s,a) = V^{\widehat{\pi},\ror}_h(s).
\end{align}
Therefore, the remainder of this step focuses on verifying the former assertion in \eqref{eq:finite-pessimism-assertion} by induction. 
\begin{itemize}
\item To begin, the claim \eqref{eq:finite-pessimism-assertion} holds at the base case when $h = H+1$, by invoking the trivial fact $\widehat{Q}_{H+1}(s,a) = Q^{\widehat{\pi},\sigma}_{H+1}(s,a) = 0$. 
\item Then, suppose that $\widehat{Q}_{h+1}(s,a) \leq Q^{\widehat{\pi},\sigma}_{h+1}(s,a)$ holds for all $(s,a)\in\cS\times \cA$ at some time step $h\in [H]$, it boils down to show $\widehat{Q}_h(s,a) \leq Q^{\widehat{\pi},\ror}_h(s,a)$. 


By the update rule of $\widehat{Q}_h(s,a)$ in Algorithm~\ref{alg:vi-lcb-dro-finite} (cf.~line~\ref{line:finite-update-Q}), the above relation holds immediately if $\widehat{Q}_h(s,a)=0$ since $\widehat{Q}_h(s,a) =0 \leq Q^{\widehat{\pi},\ror}_h(s,a)$. Otherwise, $\widehat{Q}_h(s,a)$ is updated via
\begin{align}
	\widehat{Q}_h(s,a) &= r_h(s, a)  - \widehat{\lambda}^\star_{h,s,a} \log\left(\widehat{P}_{h, s, a}   \exp \left(- \frac{\widehat{V}_{h+1}}{\widehat{\lambda}^\star_{h,s,a}}\right) \right) - \widehat{\lambda}^\star_{h,s,a} \ror - b_h(s, a) \notag\\
	& \overset{\mathrm{(i)}}{=} r_h(s, a) + \inf_{ \cP \in \unb^{\ror}(\widehat{P}_{h,s,a}^0)}   \cP \widehat{V}_{h+1} - b_h(s, a) \notag\\
	& \leq r_h(s, a) + \inf_{ \cP \in \unb^{\ror}(P_{h,s,a}^0)}  \cP \widehat{V}_{h+1}   + \left|\inf_{ \cP \in \unb^{\ror}(\widehat{P}_{h,s,a}^0)}  \cP \widehat{V}_{h+1} - \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,a})}  \cP \widehat{V}_{h+1} \right| - b_h(s,a) \notag\\
	&\overset{\mathrm{(ii)}}{\leq} r_h(s, a) + \inf_{ \cP \in \unb^{\ror}(P_{h,s,a}^0)}  \cP V^{\widehat{\pi}, \ror}_{h+1} + 0 \overset{\mathrm{(iii)}}{=}  Q^{\widehat{\pi}, \ror}_h(s,a),
\end{align}
where (i) rewrites the update rule back to its primal form (cf.~\eqref{eq:VI-primal}), (ii) holds by applying \eqref{eq:dro-b-bound} with the condition \eqref{eq:dro-b-bound-N-condition} satisfied and the induction hypothesis $\widehat{V}_{h+1} \leq V^{\widehat{\pi},\ror}_{h+1}$, and lastly, (iii) follows by the robust Bellman consistency equation \eqref{eq:robust_bellman_consistency}. 
\end{itemize}
Putting them together, we have verified the claim \eqref{eq:finite-pessimism-assertion} by induction.

\paragraph{Step 2: bounding $V_h^{\star,\ror}(s) - V^{\widehat{\pi},\ror}_{h}(s)$.} With the pessimism property \eqref{eq:finite-pessimism-assertion} in place, we observe that the following relation holds
\begin{align}
	0\leq V_h^{\star,\ror}(s) - V^{\widehat{\pi},\ror}_{h}(s) \leq V_h^{\star,\ror}(s) - \widehat{V}_{h}(s) \leq Q_h^{\star,\ror}\big(s, \pi^\star_h(s)\big) - \widehat{Q}_{h} \big(s, \pi^\star_h(s) \big),
\end{align}
where the last inequality follows from $\widehat{Q}_{h} \big(s, \pi^\star_h(s) \big) \leq \max_a \widehat{Q}_{h}  (s, a ) = \widehat{V}_{h}(s) $.
Then, by \eqref{eq:robust_bellman_optimality}
\begin{align}
	Q_h^{\star,\ror}\big(s, \pi^\star_h(s)\big) &= r_h\big(s, \pi^\star_h(s)\big) + \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP V_{h+1}^{\star,\ror},\\
	\widehat{Q}_h\big(s, \pi^\star_h(s)\big) &= r_h\big(s, \pi^\star_h(s)\big)  + \inf_{ \cP \in \unb^{\ror}(\widehat{P}_{h,s,\pi^\star_h(s)}^0)} \cP \widehat{V}_{h+1} - b_h\left(s, \pi^\star_h(s)  \right),
\end{align} 
we arrive at
\begin{align}
	V_h^{\star,\ror}(s) - \widehat{V}_{h}(s) & \leq Q_h^{\star,\ror}\big(s, \pi^\star_h(s)\big) - \widehat{Q}_{h} \big(s, \pi^\star_h(s) \big) \notag\\
	&= \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP V_{h+1}^{\star,\ror} -\inf_{ \cP \in \unb^{\ror}(\widehat{P}_{h,s,\pi^\star_h(s)}^0)}  \cP \widehat{V}_{h+1} + b_h\big(s, \pi^\star_h(s)\big) \notag\\
	& \leq \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP V_{h+1}^{\star,\ror} - \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP \widehat{V}_{h+1} \notag\\
	&\quad +\left|\inf_{\cP \in \unb^{\ror}(\widehat{P}_{h,s,a}^0)}  \cP \widehat{V}_{h+1} - \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP \widehat{V}_{h+1} \right| + b_h\big(s, \pi^\star_h(s)\big) \notag \\
	&\overset{\mathrm{(i)}}{\leq} \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP V_{h+1}^{\star,\ror} - \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}   \cP \widehat{V}_{h+1} + 2b_h\big(s, \pi^\star_h(s)\big) \notag \\
	& \overset{\mathrm{(ii)}}{\leq} \widehat{P}^{\inf}_{h,s,\pi^\star_h(s)} \big( V_{h+1}^{\star,\ror} - \widehat{V}_{h+1} \big) + 2b_h\big(s, \pi^\star_h(s) \big),\label{eq:finite-recursion-basic}
\end{align}
where (i) holds by applying \eqref{eq:dro-b-bound} with the condition \eqref{eq:dro-b-bound-N-condition} satisfied, and (ii) arises from introducing the notation 
\begin{align}
	\widehat{P}^{\inf}_{h,s,\pi^\star_h(s)} \defn \mathrm{argmin}_{\cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})} \;  \cP \widehat{V}_{h+1},
\end{align}
and consequently,
$$ \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}  \cP V_{h+1}^{\star,\ror}   \leq  \widehat{P}^{\inf}_{h,s,\pi^\star_h(s)} V_{h+1}^{\star,\ror} , \qquad \mbox{and} \qquad \inf_{ \cP \in \unb^{\ror}(P^0_{h,s,\pi^\star_h(s)})}   \cP \widehat{V}_{h+1} = \widehat{P}^{\inf}_{h,s,\pi^\star_h(s)}  \widehat{V}_{h+1}. $$

To continue, let us we introduce a sequence of matrices $\widehat{P}^{\inf}_h \in \mathbb{R}^{S\times S}$ and vectors $b_h^\star\in\mathbb{R}^S$ for $h\in[H]$, such that their $s$-th rows (resp. entries) are given by
\begin{align}
	\left[\widehat{P}^{\inf}_h \right]_{s,\cdot} = \widehat{P}^{\inf}_{h,s,\pi^\star_h(s)}, \qquad \mbox{and} \qquad  b_h^\star(s) = b_h\big(s, \pi^\star_h(s) \big).
\end{align}
With this notation in hand, applying \eqref{eq:finite-recursion-basic} recursively over the time steps $h, h+1,\cdots, H$ gives
\begin{align}
0 \leq V_h^{\star,\ror} - \widehat{V}_{h} \notag
& \leq \widehat{P}^{\inf}_{h} \big( V_{h+1}^{\star,\ror} - \widehat{V}_{h+1} \big) + 2 b_h^\star \notag\\
&\leq \widehat{P}^{\inf}_{h}\widehat{P}^{\inf}_{h+1} \big( V_{h+2}^{\star,\ror} - \widehat{V}_{h+2} \big) + 2 \widehat{P}^{\inf}_{h} b_{h+1}^\star + 2 b_h^\star \leq \cdots \leq 2 \sum_{i=h}^{H}\left(\prod_{j=h}^{i-1} \widehat{P}^{\inf}_{j}\right) b_i^\star.
\end{align}
Here, we use the notation $\left(\prod_{j=i}^{i-1} \widehat{P}^{\inf}_{j}\right) = I$ for convenience.

\yc{what is $\cD^\star_{s,h}(\ror)$?}
To continue, we denote the possible state distribution at any step $h$ associated with the optimal policy and any shifted environment as
\begin{align}
	\cD^\star_h \defn \Big\{[d_h^{\star,P}(s)]_{s\in\cS} : P \in \unb(P^{\no})\Big\} = \Big\{[d_h^{\star,P}\big(s,\pi_h^\star(s) \big)]_{s\in\cS} : P \in \unb(P^{\no})\Big\}.
\end{align}
With this in hand, it is  observed that for any $d_h^{\star} \defn = \big[d_h^{\star}(s)\big]_{s\in\cS} \in \cD^\star_h$ and any $i=h+1, \cdots, H$,
\begin{align}\label{eq:defn-of-di-star}
d_i^{\star} \defn \left[ \big(d_h^{\star}\big)^\top \left(\prod_{j=h}^{i-1} \widehat{P}^{\inf}_{j}\right)\right]^\top \in \cD^\star_i.
\end{align}
As a result, for any $d_h^{\star} \in \cD^\star_h$, we arrive at
\begin{align}\label{eq:performance-gap-h}
	\left< d_h^\star, V_h^{\star,\ror} - \widehat{V}_{h}\right> \leq \left< d_h^\star, 2 \sum_{i=h}^{H}\left(\prod_{j=h}^{i-1} \widehat{P}^{\inf}_{j}\right) b_i^\star(s) \right> \leq 2 \sum_{i=h}^H \left< d_i^\star, b_i^\star \right>.
\end{align}

\paragraph{Step 3: controlling $\left< d_i^\star, b_i^\star \right>$ using concentrability.}


Armed with Lemma~\ref{lemma:D0-property}, we shall control $\left< d_i^\star, b_i^\star \right>$ in two different cases.
\begin{itemize}
	\item When $K \myrho_i\big( (s, \pi_i^\star(s)\big) \leq 4 \cb \log\frac{KH}{\delta}$. In this case, we observe that 
	\begin{equation}
		b_i^\star(s)  \overset{\mathrm{(i)}}{\leq} H-h+1 \leq H \overset{\mathrm{(ii)}}{\leq} \frac{4\cb \Cstar H \log\frac{KH}{\delta}}{K \max_{P\in\unb(P^{\no})}\min\left\{d_i^{\star, P}\big( (s, \pi_i^\star(s)\big), \frac{1}{S}\right\}} \leq \frac{4\cb \Cstar H \log\frac{KH}{\delta}}{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\}},
	\end{equation}
	where (i) arises from the definition of $b$ in \eqref{def:bonus-dro}, (ii) follows from the definition of $\Cstar$ in \eqref{eq:concentrate-finite}, and the last inequality holds by the fact that for some $P'\in \unb(P^{\no})$(see the definition of $d_i^star$ in \eqref{eq:defn-of-di-star}),
	\begin{align}
		d_h^{\star}(s) = d_h^{\star, P'}\big( (s, \pi_i^\star(s)\big) \leq \max_{P\in\unb(P^{\no})} d_h^{\star, P}\big( (s, \pi_i^\star(s)\big).
	\end{align}

	\item When $K \myrho_i\big(s, \pi_i^\star(s)\big) > 4 \cb \log\frac{KH}{\delta}$. In such cases, applying Lemma~\ref{lemma:D0-property} with the condition assumption yields
	\begin{align}
		N_i\big(s, \pi_i^\star(s)\big) &\geq \frac{K \myrho_i\big(s, \pi_i^\star(s)\big)}{8} - 5 \sqrt{ K \myrho_h\big(s, \pi_i^\star(s)\big) \log \frac{KH}{\delta} } \geq \frac{K \myrho_i\big(s, \pi_i^\star(s)\big)}{16} \notag\\
		& = \frac{K\max_{P\in\unb(P^{\no})}\min\left\{d_i^{\star, P}\big( (s, \pi_i^\star(s)\big), \frac{1}{S}\right\}}{16 \Cstar} \geq \frac{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\}}{16 \Cstar}.
	\end{align}

With this in mind, we observe that the pessimistic penalty (see \eqref{def:bonus-dro}) obeys
	\begin{align}
		b_i^\star(s) &\leq \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{\log \frac{KH}{\delta}}{N_i\big(s, \pi_i^\star(s)\big) }} \ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) \notag \\
		&\leq \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{16 \Cstar\log \frac{KH}{\delta} }{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\} } } \ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right).
	\end{align}
\end{itemize}

Combining the results in above two cases leads to
\begin{align}
	&\sum_{s\in\cS}d_i^\star(s) b_i^\star(s) \notag \\
	&\leq \sum_{s\in\cS} d_i^\star(s) \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{16 \Cstar\log \frac{KH}{\delta} }{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\} } }\ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) + \sum_{s\in\cS} d_i^\star(s) \frac{4\cb \Cstar H \log\frac{KH}{\delta}}{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\}} \notag \\
	&\overset{\mathrm{(i)}}{\leq} \sum_{s\in\cS} d_i^\star(s) \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{16 \Cstar\log \frac{KH}{\delta} }{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\} } } \ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) +  \frac{8\cb S\Cstar H \log\frac{KH}{\delta}}{K} \notag \\
	& \overset{\mathrm{(ii)}}{\leq} \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\sum_{s\in\cS} d_i^\star(s) \frac{16 \Cstar\log \frac{KH}{\delta} }{K \min\left\{d_i^{\star}(s), \frac{1}{S}\right\} } }\sqrt{\sum_{s\in\cS} d_i^\star(s)} \ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right)+  \frac{8\cb S\Cstar H \log\frac{KH}{\delta}}{K} \notag \\
	& \leq \cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{32S \Cstar\log \frac{KH}{\delta} }{K} } \ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) +  \frac{8\cb S\Cstar H \log\frac{KH}{\delta}}{K} \label{eq:b-d-produce-bound}
\end{align}
where (i) and the last inequality hold by the trivial fact
\begin{align}\label{eq:d-star-1-S-bound}
	\sum_{s\in\cS} \frac{ d_i^\star(s)}{\min\left\{d_i^{\star}(s), \frac{1}{S}\right\}} \leq \sum_{s\in\cS} d_i^\star(s) \left(\frac{ 1}{d_i^{\star}(s)} + \frac{ 1}{1/S}\right) = \sum_{s\in\cS}1 + \frac{1}{S}\sum_{s\in\cS}d_i^\star(s) \leq 2S,
\end{align}
(ii) follows from the Cauchy-Schiwarz inequality.


Finally, inserting \eqref{eq:b-d-produce-bound} back into \eqref{eq:performance-gap-h} completes the proof by
\begin{align}
	&\left< d_h^\star, V_h^{\star,\ror} - \widehat{V}_{h}\right> \leq  2 \sum_{i=h}^H \left< d_i^\star, b_i^\star \right> \notag \\
	&\leq \sum_{i=1}^H \left(2\cb\frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{32S \Cstar\log \frac{KH}{\delta} }{K} }\ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) +  \frac{16\cb S\Cstar H \log\frac{KH}{\delta}}{K}\right) \notag \\
	& \overset{\mathrm{(i)}}{\leq} \sum_{i=1}^H \left(c_1\frac{H}{\ror} e^{\frac{4H}{\lambda_{i,s,\pi_i^\star(s)}^\star }} \sqrt{\frac{S \Cstar\log \frac{KH}{\delta} }{K} }\ind\left(\widehat{\lambda}_{i,s,\pi_i^\star(s)}^\star >0\right) +  \frac{c_1 S\Cstar H \log\frac{KH}{\delta}}{K} \right)\notag \\
	& \leq c_1\frac{H^2}{\ror} e^{\frac{4H}{\lambda^\star }} \sqrt{\frac{S \Cstar\log \frac{KH}{\delta} }{K} } +  \frac{c_1 H^2S\Cstar  \log\frac{KH}{\delta}}{K} \notag \\
\end{align}
where (i) holds by \eqref{eq:lambda-n-range} in Lemma~\ref{lem:lambda-n-bound} and $c_1$ being a large enough constant, and the last inequality holds by the definition of $\lambda^\star$ in \eqref{eq:defn-lambda-star}.


% % --------------- the upper bound version with two terms in b_h(s,a)  ---------------
% 	\begin{align}
% 		b_i^\star(s) &\leq \min\Bigg\{ \cb \frac{H}{\ror}  \sqrt{\frac{\log^2(\frac{TS}{\delta})}{ \Big(N_i\big(s, \pi_i^\star(s)\big) \widehat{\underline{p}}_h\big(s, \pi_i^\star(s)\big) \Big) \vee 1}}~,~\cb \frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{h,s, \pi_i^\star(s)}^\star }} \sqrt{\frac{\log(\frac{T}{\delta})}{N_i\big(s, \pi_i^\star(s)\big) \vee 1}} \Bigg\} \notag \\
% 		&\leq \min\Bigg\{ \cb \frac{H}{\ror}  \sqrt{\frac{16\Cstar \log^2(\frac{TS}{\delta})}{ K\min\big\{d_h^{\star}(s, a \mymid P), \frac{1}{S}\big\} \widehat{\underline{p}}_h\big(s, \pi_i^\star(s)\big) }}~,~\cb \frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{h,s, \pi_i^\star(s)}^\star }} \sqrt{\frac{16 \Cstar \log(\frac{T}{\delta})}{K\min\big\{d_h^{\star}(s, a \mymid P), \frac{1}{S}\big\} } } \Bigg\}.
% 	\end{align}
% \end{itemize}

% Combining the results in above two cases, we finally obtain
% \begin{align}
% 	&\sum_{s\in\cS}d_i^\star(s) b_i^\star(s) \notag \\
% 	&\leq \sum_{s\in\cS} d_i^\star(s) \min\Bigg\{ \cb \frac{H}{\ror}  \sqrt{\frac{16\Cstar \log^2(\frac{TS}{\delta})}{ K\min\big\{d_h^{\star}(s, a \mymid P), \frac{1}{S}\big\} \widehat{\underline{p}}_h\big(s, \pi_i^\star(s)\big) }}~,~\cb \frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{h,s, \pi_i^\star(s)}^\star }} \sqrt{\frac{16 \Cstar \log(\frac{T}{\delta})}{K\min\big\{d_h^{\star}(s, a \mymid P), \frac{1}{S}\big\} } } \Bigg\} \notag \\
% 	& \quad + \sum_{s\in\cS} d_i^\star(s) \frac{4\cb \Cstar H \log\frac{TH}{\delta}}{K \min\big\{d_h^{\star}(s, a \mymid P), \frac{1}{S}\big\}} \notag \\
% 	&\leq \min \Bigg\{ \cb \frac{H}{\ror}  \sqrt{\frac{S \Cstar \log^2(\frac{TS}{\delta})}{ K \widehat{\underline{p}}_h\big(s, \pi_i^\star(s)\big) }}~,~\cb \frac{H}{\ror} e^{\frac{2H}{\widehat{\lambda}_{h,s, \pi_i^\star(s)}^\star }} \sqrt{\frac{S\Cstar \log(\frac{T}{\delta})}{K } }\Bigg\} + \frac{\cb HS\Cstar \log\frac{TH}{\delta}}{K }.
% \end{align}

% Finally, we arrive at
% \begin{align}
% 	&\left< d_h^\star, V_h^\star - \widehat{V}_{h}\right> \leq  2 \sum_{i=h}^H \left< d_i^\star, b_i^\star \right> \notag \\
% 	&\leq \min \Bigg\{ \cb \frac{H^2}{\ror}  \sqrt{\frac{S \Cstar \log^2(\frac{TS}{\delta})}{ K \widehat{\underline{p}}_h\big(s, \pi_i^\star(s)\big) }}~,~\cb \frac{H^2}{\ror} e^{\frac{2H}{\widehat{\lambda}_{h,s, \pi_i^\star(s)}^\star }} \sqrt{\frac{S\Cstar \log(\frac{T}{\delta})}{K } }\Bigg\} + \frac{\cb H^2S\Cstar \log\frac{TH}{\delta}}{K }.
% \end{align}
% \lxs{transfer from $\widehat{p}, \widehat{\lambda}$ to $p, \lambda$.}
% % --------------- the upper bound version with two terms in b_h(s,a) above ---------------

